Contextual Linear Types for Differential Privacy

Language support for differentially-private programming is both crucial and delicate. While elaborate program logics can be very expressive, type-system based approaches using linear types tend to be more lightweight and amenable to automatic checking and inference, and in particular in the presence of higher-order programming. Since the seminal design of Fuzz, which is restricted to $\epsilon$-differential privacy in its original design, significant progress has been made to support more advancedvariants of differential privacy, like($\epsilon$,$\delta$)-differential privacy. However, supporting these advanced privacy variants while also supporting higher-order programming in full has proven to be challenging. We present Jazz, a language and type system which uses linear types and latent contextual effects to support both advanced variants of differential privacy and higher-order programming. Latent contextual effects allow delaying the payment of effects for connectives such as products, sums and functions, yielding advantages in terms of precision of the analysis and annotation burden upon elimination, as well as modularity. We formalize the core of Jazz, prove it sound for privacy via a logical relation for metric preservation, and illustrate its expressive power through a number of case studies drawn from the recent differential privacy literature.

==> sensitivity-dynamic-semantics.tex <==
\begin{framed}
\begingroup\color{\colorMATH}\begin{gather*}\begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\begin{array}{rclcl@{\hspace*{1.00em}}l
} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } &{}\in {}& {\text{val}}   &{}\mathrel{\Coloneqq }{}& {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{r}}}\endgroup }  \mathrel{|} \langle \lambda x:\tau  \mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup } .\hspace*{0.33em}e,\gamma \rangle  \mathrel{|} \ttt \mathrel{|} \inl\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } \mathrel{|} \inr\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } \mathrel{|} \addProduct{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv_{1}}}}\endgroup }}{ {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv_{2}}}}\endgroup }}  \cr    &{} {}&  &{}\mathrel{|}{}& \langle {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv_{1}}}}\endgroup },{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv_{2}}}}\endgroup }\rangle                  & {{\color{\colorTEXT}\textnormal{values}}}
\cr  \gamma  &{}\in {}& {\text{venv}}  &{}\triangleq {}& {\text{var}} \rightharpoonup  {\text{val}} \mathrel{\Coloneqq } \{ x\mapsto {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup },\ldots ,x\mapsto {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }\}                                               & {{\color{\colorTEXT}\textnormal{value environment}}}
\end{array}
\end{tabularx}
\end{gather*}\endgroup
\begingroup\color{\colorMATH}\begin{gather*}
\begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\parbox{\linewidth}{
\begingroup\color{\colorMATH}\begin{mathpar} \inferrule*[lab={\textsc{ rlit}}
   ]{ }{
      \gamma \vdash {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{r}}}\endgroup } \Downarrow ^{0} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{r}}}\endgroup }
   }
\and \inferrule*[lab={\textsc{ plus}}
   ]{ \gamma \vdash {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }  \Downarrow ^{k_{1}} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{r}}}\endgroup } 
   \\ \gamma \vdash {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }  \Downarrow ^{k_{2}} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{r}}}\endgroup } 
      }{
      \gamma \vdash {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } +{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }  \Downarrow ^{k_{1}+k_{2}+1} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{r}}}\endgroup } +{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{r}}}\endgroup } 
   }
\and \inferrule*[lab={\textsc{ times}}
   ]{ \gamma \vdash {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }  \Downarrow ^{k_{2}} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{r}}}\endgroup } 
   \\ \gamma \vdash {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }  \Downarrow ^{k_{2}} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{r}}}\endgroup } 
      }{
      \gamma \vdash {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }  \Downarrow ^{k_{1}+k_{2}+1} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{r}}}\endgroup } {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{r}}}\endgroup } 
   }
\and \inferrule*[lab={\textsc{ leq}}
   ]{ \gamma \vdash {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }  \Downarrow ^{k_{1}} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{r}}}\endgroup } 
   \\ \gamma \vdash {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }  \Downarrow ^{k_{2}} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{r}}}\endgroup } 
      }{
      \gamma \vdash {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \leq {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }  \Downarrow ^{k_{1}+k_{2}+1} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{r}}}\endgroup } \leq {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{r}}}\endgroup } 
   }
\and \inferrule*[lab={\textsc{ var}}
   ]{ \gamma (x) = {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }
      }{
      \gamma \vdash x \Downarrow ^{1} v
   }
\and \inferrule*[lab={\textsc{ lam}}
   ]{ \gamma ' \subseteq  \gamma 
   \\ FV({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }) = dom(\gamma ')
      }{
      \gamma \vdash {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\slambda}}}\endgroup } (x\mathrel{:}\tau  \mathord{\cdotp } {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }).\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \Downarrow ^{1} \langle {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\slambda}}}\endgroup } x:\tau \mathord{\cdotp } {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }.\hspace*{0.33em}e, \gamma \rangle 
   }
\and \inferrule*[lab={\textsc{ app}}
   ]{ \gamma \vdash {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }  \Downarrow ^{k_{1}} \langle \lambda x:\tau \mathord{\cdotp } {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }.\hspace*{0.33em}e^{\prime},\gamma ^{\prime}\rangle 
   \\ \gamma \vdash {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }  \Downarrow ^{k_{2}} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } 
   \\ \gamma ^{\prime}[x\mapsto {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } ]\vdash e^{\prime} \Downarrow ^{k_{3}} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } 
      }{
      \gamma \vdash {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }  \Downarrow ^{k_{1}+k_{2}+k_{3}+1} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } 
   }
\and \inferrule*[lab={\textsc{ unit}}
   ]{ }{
      \gamma \vdash {{\color{\colorSYNTAX}\texttt{tt}}} \Downarrow ^{0} {{\color{\colorSYNTAX}\texttt{tt}}}
   }
\and \inferrule*[lab={\textsc{ inl}}
   ]{ \gamma \vdash {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \Downarrow ^{k} v
      }{
      \gamma \vdash \inl^{\tau _{2}}\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \Downarrow ^{k} \inl\hspace*{0.33em}v
   }
\and \inferrule*[lab={\textsc{ inr}}
   ]{ \gamma \vdash {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \Downarrow ^{k} v
      }{
      \gamma \vdash \inr^{\tau _{1}}\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \Downarrow ^{k} \inr\hspace*{0.33em}v
   }
\and \inferrule*[lab={\textsc{ case-left}}
   ]{ \gamma \vdash {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }  \Downarrow ^{k_{1}} \inl\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } 
   \\ \gamma [x\mapsto {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } ]\vdash {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }  \Downarrow ^{k_{2}} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } 
      }{
      \gamma \vdash \ccase\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }\hspace*{0.33em}\of\hspace*{0.33em}\{ x\Rightarrow {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \} \hspace*{0.33em}\{ x\Rightarrow e_{3}\}  \Downarrow ^{k_{1}+k_{2}+1} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } 
   }
\and \inferrule*[lab={\textsc{ case-right}}
   ]{ \gamma \vdash {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }  \Downarrow ^{k_{1}} \inr\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } 
   \\ \gamma [x\mapsto {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } ]\vdash e_{3} \Downarrow ^{k_{2}} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } 
      }{
      \gamma \vdash \ccase\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }\hspace*{0.33em}\of\hspace*{0.33em}\{ x\Rightarrow {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \} \hspace*{0.33em}\{ x\Rightarrow e_{3}\}  \Downarrow ^{k_{1}+k_{2}+1} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } 
   }
\and \inferrule*[lab={\textsc{ pair}}
   ]{ \gamma \vdash {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }  \Downarrow ^{k_{1}} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } 
   \\ \gamma \vdash {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }  \Downarrow ^{k_{2}} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } 
      }{
      \gamma \vdash \addProduct{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }}{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } } \Downarrow ^{k_{1}+k_{2}} \addProduct{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }}{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } }
   }
\and \inferrule*[lab={\textsc{ proj1}}
   ]{ \gamma \vdash {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \Downarrow ^{k} \addProduct{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }}{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } }
      }{
      \gamma \vdash \fst\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \Downarrow ^{k+1} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } 
   }
\and \inferrule*[lab={\textsc{ proj2}}
   ]{ \gamma \vdash {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \Downarrow ^{k} \addProduct{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }}{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } }
      }{
      \gamma \vdash \snd\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \Downarrow ^{k+1} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } 
   }
\and \inferrule*[lab={\textsc{ tup}}
  ]{ \gamma \vdash {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }  \Downarrow ^{k_{1}} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } 
  \\ \gamma \vdash {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }  \Downarrow ^{k_{2}} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } 
     }{
     \gamma \vdash \langle {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } ,{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \rangle  \Downarrow ^{k_{1}+k_{2}} \langle {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } ,{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } \rangle 
  }
\and \inferrule*[lab={\textsc{ untup}}
   ]{ \gamma \vdash {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }  \Downarrow ^{k_{1}} \langle {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } ,{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } \rangle 
   \\ \gamma [x_{1}\mapsto {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } ,x_{2}\mapsto {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } ] \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }  \Downarrow ^{k_{2}} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } ^{\prime}
      }{
      \gamma \vdash \tlet\hspace*{0.33em}x_{1},x_{2}={\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \hspace*{0.33em}\tin\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }  \Downarrow ^{k_{1}+k_{2}+1} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } ^{\prime}
   }
\and \inferrule*[lab={\textsc{ ascr}}
   ]{ \gamma \vdash {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \Downarrow ^{k} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }
      }{
      \gamma \vdash {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } :: {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\tau }}}\endgroup } \Downarrow ^{k+1} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }
   }
\end{mathpar}\endgroup
}
% \cr  \hfill\hspace{0pt}{{\color{\colorTEXT}\textnormal{{\textit{\ldots  derived rules}}}}}
% \cr \parbox{\linewidth}{
% \begingroup\color{\colorMATH}\begin{mathpar} \inferrule*[lab={\textsc{ blit}}
%    ]{ }{
%       \gamma \vdash b \Downarrow  b
%    }
% \and \inferrule*[lab={\textsc{ if-true}}
%    ]{ \gamma \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \Downarrow  {\text{true}}
%    \\ \gamma \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup } \Downarrow  v
%       }{
%       \gamma \vdash {{\color{\colorSYNTAX}\texttt{if}}}\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \hspace*{0.33em}\{ {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \} \hspace*{0.33em}\{ e_{3}\}  \Downarrow  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }
%    }
% \and \inferrule*[lab={\textsc{ if-false}}
%    ]{ \gamma \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }  \Downarrow  {\text{false}}
%    \\ \gamma \vdash  e_{3} \Downarrow  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }
%       }{
%       \gamma \vdash {{\color{\colorSYNTAX}\texttt{if}}}\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \hspace*{0.33em}\{ {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \} \hspace*{0.33em}\{ e_{3}\}  \Downarrow  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }
%    }
% \and \inferrule*[lab={\textsc{ let}}
%    ]{ \gamma \vdash {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }  \Downarrow  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } 
%    \\ \gamma [x\mapsto {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } ] \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }  \Downarrow  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } 
%       }{
%       \gamma \vdash \tlet\hspace*{0.33em}x={\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \hspace*{0.33em}\tin\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }  \Downarrow  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } 
%    }
% \end{mathpar}\endgroup
% }
\end{tabularx}
\end{gather*}\endgroup
\end{framed}

==> statics-auxiliary-definitions.tex <==
\begin{framed}
\begingroup\color{\colorMATH}\begin{gather*}
  \begin{tabularx}{\linewidth}{>{\centering\arraybackslash\(}X<{\)}}\hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup }/x]\tau  \endgroup}\endgroup %{{\color{\colorTEXT}\textnormal{{\textit{Sensitivity environment substitution}}}}}
  \cr \begin{array}{rcl
    } [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup }/x]{\mathbb{R}} &{}={}& {\mathbb{R}}
    \cr  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup }/x]((y\mathrel{:}\tau _{1} \mathord{\cdotp } {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }) \xrightarrow {{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'}}}\endgroup }} \tau _{2}) &{}={}& (y\mathrel{:}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup }/x]\tau _{1} \mathord{\cdotp } {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }) \xrightarrow {[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'}}}\endgroup }} [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup }/x]\tau _{2}
    \cr  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup }/x](\tau _{1} \mathrel{^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}\oplus ^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }}} \tau _{2}) &{}={}& [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup }/x]\tau _{1} \mathrel{^{[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}\oplus ^{[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }}} [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup }/x]\tau _{2}
    \end{array}
  \cr \hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup } \endgroup}\endgroup%[\_/x]\_: {\text{sensv}} \times  {\text{sensv}} \rightarrow  {\text{sensv}}
  \cr \begin{array}{rcl
    } [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup }/x]\varnothing  &{}={}& \varnothing 
    \cr  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup }/x]({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }x) &{}={}& [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup }
    \cr  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup }/x]({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }y) &{}={}& [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }y
    \end{array}
  \cr \hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \tau  \sqcup  \tau  \endgroup}\endgroup
  \cr \begin{array}{rcl
    } {\mathbb{R}} \sqcup  {\mathbb{R}} &{}={}& {\mathbb{R}}
    \cr  (y\mathrel{:}\tau _{1} \mathord{\cdotp } {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }) \xrightarrow {{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup }} \tau _{1} \sqcup  (y\mathrel{:}\tau '_{1} \mathord{\cdotp } {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'}}}\endgroup }) \xrightarrow {{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'}}}\endgroup }} \tau '_{2} &{}={}& (y\mathrel{:}\tau _{1} \sqcap  \tau '_{1} \mathord{\cdotp } {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup } \sqcap  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'}}}\endgroup }) \xrightarrow {{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup } \sqcup  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'}}}\endgroup }} (\tau _{2} \sqcup  \tau '_{2})
    \cr  \tau _{1} \mathrel{^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}\oplus ^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }}} \tau _{2} \sqcup  (\tau '_{1} \mathrel{^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup }}\oplus ^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup }}} \tau '_{2}) &{}={}& (\tau _{1} \sqcup  \tau '_{1}) \mathrel{^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup } \sqcup  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup }}\oplus ^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup } \sqcup  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup }}} (\tau _{2} \sqcup  \tau '_{2})
    \end{array}
  \cr \hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup } \sqcup  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup } \endgroup}\endgroup %\_ \sqcup  \_: {\text{sensv}} \times  sensv  \rightarrow  sensv
  \cr \begin{array}{rclr
    } \varnothing  \sqcup  \varnothing  &{}={}& \varnothing 
    \cr  ({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }x) \sqcup  ({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'}}}\endgroup }x) &{}={}& ({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup } \sqcup  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'}}}\endgroup }) + ({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup } \sqcup  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'}}}\endgroup })x & {{\color{\colorTEXT}\textnormal{ ({{\color{\colorMATH}\ensuremath{x \notin  dom({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup } \sqcup  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'}}}\endgroup })}}})}}}
    \cr  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup } \sqcup  ({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }x) = ({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }x) \sqcup  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup } &{}={}& ({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup } \sqcup  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'}}}\endgroup }) + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }x & {{\color{\colorTEXT}\textnormal{ ({{\color{\colorMATH}\ensuremath{x \notin  dom({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup })}}})}}}
    \end{array}
	\cr \hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup } <: {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup } \endgroup}\endgroup
	\cr \hfill\hspace{0pt}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup } <: {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS^{\prime}}}}\endgroup } \overset \vartriangle \iff     \forall x.\hspace*{0.33em} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup }(x) \leq  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS^{\prime}}}}\endgroup }(x)
	  \hfill\hspace{0pt}
	\cr \hfill\hspace{0pt}\begingroup\color{\colorTEXT}\boxed{\begingroup\color{\colorMATH} \tau  <: \tau  \endgroup}\endgroup
	\cr \parbox{\linewidth}{
	\begingroup\color{\colorMATH}\begin{mathpar}\inferrule*[lab={\textsc{ base}}
	  ]{ \tau  \in  \{ {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorSYNTAX}\texttt{{\ensuremath{{\mathbb{R}}}}}}}\endgroup },{{\color{\colorSYNTAX}\texttt{unit}}}\} 
	     }{
	     \tau  <: \tau 
	  }
	\and\inferrule*[lab={\textsc{ s-lam}}
	  ]{ \tau _{1}^{\prime} <: \tau _{1}
	  \\ {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'}}}\endgroup } <: {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }
	  \\ {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup } <: {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS^{\prime}}}}\endgroup }
	  \\ \tau _{2} <: \tau _{2}^{\prime}
	     }{
	     (x:\tau _{1} \mathord{\cdotp } {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }) \overset {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup }\rightarrow  \tau _{2} \hspace*{0.33em}<:\hspace*{0.33em} (x:\tau _{1}^{\prime} \mathord{\cdotp } {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'}}}\endgroup }) \oversetcustom{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS^{\prime}}}}\endgroup }}\rightarrow   \tau _{2}^{\prime}
	  }
	\and\inferrule*[lab={\textsc{ sum}}
	  ]{ \tau _{1} <: \tau _{1}^{\prime}
	  \\ {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup } <: {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}^{\prime}}}}\endgroup }
	  \\ \tau _{2} <: \tau _{2}^{\prime}
	  \\ {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup } <: {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}^{\prime}}}}\endgroup }
	     }{
	     \tau _{1} \mathrel{^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}\oplus ^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }}} \tau _{2} \hspace*{0.33em}<:\hspace*{0.33em} \tau _{1}^{\prime} \mathrel{^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}^{\prime}}}}\endgroup }}\oplus ^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}^{\prime}}}}\endgroup }}} \tau _{2}^{\prime}
	  }
	% \and\inferrule*[lab={\textsc{ pair}}
	%   ]{ \tau _{1} <: \tau _{1}^{\prime}
	%   \\ {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup } <: {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}^{\prime}}}}\endgroup }
	%   \\ \tau _{2} <: \tau _{2}^{\prime}
	%   \\ {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup } <: {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}^{\prime}}}}\endgroup }
	%      }{
	%      \tau _{1} \mathrel{^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}\&^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }}} \tau _{2} \hspace*{0.33em}<:\hspace*{0.33em} \tau _{1}^{\prime} \mathrel{^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}^{\prime}}}}\endgroup }}\&^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}^{\prime}}}}\endgroup }}} \tau _{2}^{\prime}
	%   }
	\end{mathpar}\endgroup
	}
	\end{tabularx}
\end{gather*}\endgroup
\end{framed}


==> type-preservation.tex <==
Let us prove type safety for $\lang$.
We first define two operators to remove variables from a type, which will be use throughout this section.

$$\tau /\Gamma  = [\varnothing /x_{1},...,\varnothing /x_{n}]\tau , \forall  x_{i} \in  dom(\Gamma )$$
$$\tau /\gamma  = [\varnothing /x_{1},...,\varnothing /x_{n}]\tau , \forall  x_{i} \in  dom(\gamma )$$

Next we present the type rule for closures which will be used in the type preservation lemma:
 \begingroup\color{\colorMATH}\begin{gather*} 
	\inferrule*[lab={\textsc{ closure}}
	]{ \exists \Gamma ', {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{0}}}}\endgroup }, dom({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS''}}}\endgroup }) \subseteq  dom(\Gamma ') \subseteq  dom({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{0}}}}\endgroup }) 
	\\ \forall  x_{i} \in  dom(\Gamma '), \varnothing ; \varnothing  \vdash  \gamma (x_{i}) : \tau '_{i}, \tau '_{i} <: \Gamma '(x_{i}) ; \varnothing 
	\\ \Gamma ', x: \tau _{1}; {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{0}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss_{1}}}}\endgroup }x \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se'}}}\endgroup } \mathrel{:} \tau _{2} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS''}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'}}}\endgroup }x
	  }{
	  \Gamma ; {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \vdash  \langle {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\slambda}}}\endgroup } (x\mathrel{:}\tau _{1}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss_{1}}}}\endgroup }).\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se'}}}\endgroup }, \gamma \rangle  \mathrel{:} (x\mathrel{:} \tau _{1}/\Gamma '\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss_{1}}}}\endgroup }) \xrightarrow {{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'}}}\endgroup }x} \tau _{2}/\Gamma ' \mathrel{;} \varnothing 
	}
\end{gather*}\endgroup

To define type preservation of the privacy language, we define a non-deterministic sampling semantics of privacy expressions in Figure~\ref{afig:interpreter-prob-sem-tp}.

\begin{figure}[t]
\begin{small}
\begin{framed}
\begingroup\color{\colorMATH}\begin{mathpar}\inferrule*[lab={\textsc{ return}}
  ]{ \gamma  \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \Downarrow  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }
    }{
     {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorSYNTAX}\texttt{return}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \Downarrow  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }
  }
\and\inferrule*[lab={\textsc{ bind}}
  ]{ \Gamma  \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{1}}}}\endgroup } \mathrel{:} \tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{1}}}}\endgroup }
  \\ \Gamma ,x\mathrel{:}\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{0}}}\endgroup }x   \hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{2}}}}\endgroup } \mathrel{:} \tau _{2} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{2}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{p}}}\endgroup }{\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{x}}}\endgroup }
    }{
     \Gamma  \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em} x: \tau _{1} \leftarrow  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{1}}}}\endgroup }\mathrel{;}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{2}}}}\endgroup } \mathrel{:} [\varnothing /x]\tau _{2} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{2}}}}\endgroup }
  }
\and\inferrule*[lab={\textsc{ if}}
  ]{ \Gamma  \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \mathrel{:} {\mathbb{B}} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }
  \\ \Gamma  \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }   \hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{2}}}}\endgroup } \mathrel{:} \tau  \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{2}}}}\endgroup }
  \\ \Gamma  \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }   \hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{3}}}}\endgroup } \mathrel{:} \tau  \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{3}}}}\endgroup }
     }{
     \Gamma  \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em} if\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }\hspace*{0.33em}\{ {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{2}}}}\endgroup }\} \hspace*{0.33em}\{ {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{3}}}}\endgroup }\}  \mathrel{:} \tau  \mathrel{;}  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}}}\endgroup }\lceil ^{\infty }}}}\endgroup } + ({\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{2}}}}\endgroup } \sqcup  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{3}}}}\endgroup })
  }
\and \inferrule*[lab={\textsc{ p-case}}
   ]{ \Gamma  \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \mathrel{:} \tau _{1 1} \mathrel{^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1 1}}}}\endgroup }}\oplus ^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1 2}}}}\endgroup }}} \tau _{1 2} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }
   \\ \Gamma ,x\mathrel{:}\tau _{1 1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } + ({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \mathord{\cdotp } ({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1 1}}}}\endgroup }))x   \hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{2}}}}\endgroup } \mathrel{:} \tau _{2} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{2}}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{p_{2}}}}\endgroup }x
   \\ \Gamma ,y\mathrel{:}\tau _{1 2} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } + ({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \mathord{\cdotp } ({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1 2}}}}\endgroup }))y   \hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{3}}}}\endgroup } \mathrel{:} \tau _{3} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{3}}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{p_{3}}}}\endgroup }y
      }{
      \Gamma  \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em} {{\color{\colorSYNTAX}\texttt{case}}}\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{of}}}\hspace*{0.33em}\{ x\Rightarrow {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{2}}}}\endgroup }\} \hspace*{0.33em}\{ y\Rightarrow {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{3}}}}\endgroup }\}  \mathrel{:} \qquad\qquad\qquad\qquad\qquad\qquad
    \\ \qquad\qquad\qquad [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1 1}}}}\endgroup }/x]\tau _{2} \sqcup  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1 2}}}}\endgroup }/y]\tau _{3} \mathrel{;}  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \times  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}}}\endgroup }\lceil ^{\infty }}}}\endgroup } + (( {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1 1}}}}\endgroup }\lceil ^{p_{2}}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{2}}}}\endgroup }) \sqcup  ( {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1 2}}}}\endgroup }\lceil ^{p_{3}}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{3}}}}\endgroup }))
   }
\and \inferrule*[lab={\textsc{ p-app}}
  ]{ \Gamma  \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \mathrel{:} (x\mathrel{:}\tau _{1}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }) \xrightarrow {{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{p}}}\endgroup }x} \tau _{2} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }
  \\ \Gamma  \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup } \mathrel{:} \tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }
  \\ {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \mathord{\cdotp } {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup } \leq  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }
     }{
     \Gamma  \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{1}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{2}}}}\endgroup } \mathrel{:} [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }/x]\tau _{2} \mathrel{;}  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \times  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}}}\endgroup }\lceil ^{\infty }}}}\endgroup } +  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \times  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }}}}\endgroup }\lceil ^{p}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS}}}\endgroup }
  }
\end{mathpar}\endgroup
\end{framed}
\end{small}
\label{afig:interpreter-prob-sem-tp}
\caption{Interpreter for probabilistic expressions}
\end{figure}

\begin{small}
\begin{framed}
\begingroup\color{\colorMATH}\begin{mathpar}
   \inferrule*[lab={\textsc{ }}
   ]{ \varnothing ; \varnothing  \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } : \tau '; \varnothing 
   \\  \tau ' <: \tau 
      }{
      {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } \in  Atom\llbracket \tau \rrbracket 
   }
\and \inferrule*[lab={\textsc{ }}
   ]{ dom(\Gamma ) = dom(\gamma ) 
   \\ \forall  x \in  dom(\gamma ). 
   \\ \gamma (x) \in  {\mathcal{V}}^{k}\llbracket \Gamma (x)/\Gamma \rrbracket  
      }{
      \gamma  \in  {\mathcal{G}}^{k}\llbracket \Gamma \rrbracket 
   }
\and \inferrule*[lab={\textsc{ }}
   ]{ \varnothing ; \varnothing  \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{r}}}\endgroup } \in  Atom\llbracket {\mathbb{R}}\rrbracket 
      }{
      {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{r}}}\endgroup } \in  {\mathcal{V}}^{k}\llbracket {\mathbb{R}}\rrbracket 
   }	
\and \inferrule*[lab={\textsc{ }}
   ]{ \varnothing ; \varnothing  \vdash  \langle {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\slambda}}}\endgroup } x:\tau \mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }. {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }, \gamma \rangle  \in  Atom\llbracket (x\mathrel{:}\tau _{1}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }) \xrightarrow {{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }} \tau _{2}\rrbracket 
   \\ \forall   {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } \in  {\mathcal{V}}^{k}\llbracket \tau _{1}\rrbracket . \gamma [x \mapsto  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }] \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \in  {\mathcal{E}}^{k}\llbracket \tau _{2}\rrbracket 
      }{
      \langle {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\slambda}}}\endgroup } x:\tau \mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }. {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }, \gamma \rangle  \in  {\mathcal{V}}^{k}\llbracket (x\mathrel{:}\tau _{1}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }) \xrightarrow {{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }} \tau _{2}\rrbracket 
   }
\and \inferrule*[lab={\textsc{ }}
   ]{ \varnothing ; \varnothing  \vdash  \langle {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\slambda}}}\endgroup } x:\tau \mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }. {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe}}}\endgroup }, \gamma \rangle  \in  Atom\llbracket (x\mathrel{:}\tau _{1}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }) \xrightarrow {{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{1}}}}\endgroup }} \tau _{2}\rrbracket 
   \\ \forall   {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } \in  {\mathcal{V}}\llbracket \tau _{1}\rrbracket . \gamma [x \mapsto  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }] \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe}}}\endgroup } \in  {\mathcal{E}}\llbracket \tau _{2}\rrbracket 
      }{
      \langle {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\slambda}}}\endgroup } x:\tau \mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }. {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe}}}\endgroup }, \gamma \rangle  \in  {\mathcal{V}}^{k}\llbracket (x\mathrel{:}\tau _{1}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }) \xrightarrow {{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{1}}}}\endgroup }} \tau _{2}\rrbracket 
   }
\and \inferrule*[lab={\textsc{ }}
   ]{ 
   \gamma  \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \Downarrow  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }
   \\  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } \in  {\mathcal{V}}\llbracket \tau \rrbracket 
      }{
      \gamma  \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \in  {\mathcal{E}}\llbracket \tau \rrbracket 
   }
\and \inferrule*[lab={\textsc{ }}
   ]{ 
   \gamma  \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe}}}\endgroup } \Downarrow  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }
   \\  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } \in  {\mathcal{V}}\llbracket \tau \rrbracket 
      }{
      \gamma  \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe}}}\endgroup } \in  {\mathcal{E}}\llbracket \tau \rrbracket 
   }
\end{mathpar}\endgroup
\end{framed}
\end{small}

% \begin{proposition}[Fundamental Property]
%   \label{lm:type-safety-FP}
%   Let {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }; \Gamma  \vdash 	{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } : \tau  ; {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup }}}}, and {{\color{\colorMATH}\ensuremath{\gamma  \in  {\mathcal{G}}\llbracket \Gamma \rrbracket }}}.
%   Then {{\color{\colorMATH}\ensuremath{\gamma \vdash {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \in  {\mathcal{E}}\llbracket \tau /\Gamma \rrbracket }}}.
% \end{proposition}
\begin{proposition}[Fundamental Property]
  \label{lm:type-safety-FP}\;
  \begin{enumerate}\item  Let {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }; \Gamma  \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } : \tau  ; {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup }}}}, and {{\color{\colorMATH}\ensuremath{\gamma  \in  {\mathcal{G}}\llbracket \Gamma \rrbracket }}}. Then
		{{\color{\colorMATH}\ensuremath{\gamma \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \in  {\mathcal{E}}\llbracket \tau /\Gamma \rrbracket }}}.
  \item  Let {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }; \Gamma  \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe}}}\endgroup } : \tau  ; {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS}}}\endgroup }}}}, and {{\color{\colorMATH}\ensuremath{\gamma  \in  {\mathcal{G}}\llbracket \Gamma \rrbracket }}}.  Then
		{{\color{\colorMATH}\ensuremath{\gamma \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe}}}\endgroup } \in  {\mathcal{E}}\llbracket \tau /\Gamma \rrbracket }}}.
  \end{enumerate}
\end{proposition}
\begin{proof}
Let us prove first (1).
We proceed by induction on {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }; \Gamma  \vdash 	{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } : \tau  ; {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup }}}}.
\begin{enumerate}[ncases]\item  {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }; \Gamma  \vdash 	x : \Gamma (x) ; x}}}
	\begin{subproof} 
	 By {{\color{\colorMATH}\ensuremath{\gamma  \in  {\mathcal{G}}\llbracket \Gamma \rrbracket }}}, we know that {{\color{\colorMATH}\ensuremath{\gamma (x) \in  {\mathcal{V}}\llbracket \Gamma (x)/\Gamma \rrbracket }}} . By inspection of the reduction rules, we know that
	 {{\color{\colorMATH}\ensuremath{\gamma  \vdash  x \Downarrow ^{1} \gamma (x)}}}. We have to prove that {{\color{\colorMATH}\ensuremath{\gamma (x) \in  {\mathcal{V}}\llbracket \Gamma (x)/\Gamma \rrbracket }}}, which we already know and the result holds.
	\end{subproof}
\item  {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }; \Gamma  \vdash 	 {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{r}}}\endgroup } : {\mathbb{R}} ; \varnothing }}}
	\begin{subproof} 
	 Trivial as {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{r}}}\endgroup } \in  {\mathcal{V}}\llbracket {\mathbb{R}}\rrbracket }}}. 
	\end{subproof}
\item  {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }; \Gamma  \vdash 	{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup } : \tau  ; {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup }}}}
	\begin{subproof} 
	By {{\color{\colorMATH}\ensuremath{{\textsc{ s-app}}}}} we know that
	\begingroup\color{\colorMATH}\begin{gather*} 
	   \inferrule*[lab={\textsc{ s-app}}
	   ]{ \Gamma  \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \mathrel{:} (x\mathrel{:}\tau _{1}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss_{1}}}}\endgroup }) \xrightarrow {{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss_{2}}}}\endgroup }x } \tau _{2} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }
	   \\ \Gamma  \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup } \mathrel{:} \tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }
	   \\ {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup } \leq  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss_{1}}}}\endgroup }
	      }{
	      \Gamma  \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup } \mathrel{:} [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }/x]\tau _{2} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss_{2}}}}\endgroup }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'}}}\endgroup }
	   }
	\end{gather*}\endgroup
	where {{\color{\colorMATH}\ensuremath{\tau  = [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }/x]\tau _{2}}}}, and {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup } = {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss_{2}}}}\endgroup }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'}}}\endgroup }}}}.
	By induction hypotheses we know that {{\color{\colorMATH}\ensuremath{\exists  k_{1},k_{2}, j_{1}, j_{2}}}},
	{{\color{\colorMATH}\ensuremath{\gamma  \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \Downarrow ^{j_{1}} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv_{1}}}}\endgroup }}}}, {{\color{\colorMATH}\ensuremath{\gamma  \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup } \Downarrow ^{j_{2}} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv_{2}}}}\endgroup }}}},
	% {{\color{\colorMATH}\ensuremath{\varnothing ; \varnothing  \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv_{1}}}}\endgroup }: (x\mathrel{:}\tau '_{1}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'_{1}}}}\endgroup }) \xrightarrow {{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS''}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'_{2}}}}\endgroup }x } \tau '_{2} ; \varnothing }}}, {{\color{\colorMATH}\ensuremath{\varnothing ; \varnothing  \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv_{2}}}}\endgroup }: \tau '''_{1} ; \varnothing }}}, such that 
	% {{\color{\colorMATH}\ensuremath{(x\mathrel{:}\tau '_{1}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'_{1}}}}\endgroup }) \xrightarrow {{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS''}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'_{2}}}}\endgroup }x } \tau '_{2} <: (x\mathrel{:}\tau _{1}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss_{1}}}}\endgroup }) \xrightarrow {{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss_{2}}}}\endgroup }x } \tau _{2}}}} (i.e. {{\color{\colorMATH}\ensuremath{\tau _{1} <: \tau '_{1}, {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss_{1}}}}\endgroup } <: {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'_{1}}}}\endgroup }, {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS''}}}\endgroup } <: {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'}}}\endgroup }, {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'_{2}}}}\endgroup } \leq  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss_{2}}}}\endgroup }}}}, and {{\color{\colorMATH}\ensuremath{\tau '_{2} <: \tau _{2}}}}), and 
	% {{\color{\colorMATH}\ensuremath{\tau '''_{1} <: \tau _{1}}}}.
	{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv_{1}}}}\endgroup } \in  {\mathcal{V}}^{k_{1}}\llbracket (x\mathrel{:}\tau _{1}/\Gamma \mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss_{1}}}}\endgroup }) \xrightarrow {{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss_{2}}}}\endgroup }x } \tau _{2}/\Gamma \rrbracket }}} and 
	{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv_{2}}}}\endgroup } \in  {\mathcal{V}}^{k_{2}}\llbracket \tau _{1}/\Gamma \rrbracket }}}.

	By inspection of the function predicate, we know that 
	{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv_{1}}}}\endgroup } \in  Atom\llbracket (x\mathrel{:}\tau _{1}/\Gamma \mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss_{1}}}}\endgroup }) \xrightarrow {{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss_{2}}}}\endgroup }x } \tau _{2}/\Gamma \rrbracket }}} and 
	{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv_{1}}}}\endgroup } = \langle {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\slambda}}}\endgroup } (x\mathrel{:}\tau '_{1}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'_{1}}}}\endgroup }).\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se'}}}\endgroup }, \gamma '\rangle }}}, for some {{\color{\colorMATH}\ensuremath{\tau '_{1}, {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'_{1}}}}\endgroup }, {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se'}}}\endgroup }}}} and {{\color{\colorMATH}\ensuremath{\gamma '}}}.
	We also know then that 
	{{\color{\colorMATH}\ensuremath{\gamma '[x \mapsto  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv_{2}}}}\endgroup }] \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se'}}}\endgroup } \in  {\mathcal{E}}\llbracket \tau _{2}/\Gamma \rrbracket }}}, i.e.
	{{\color{\colorMATH}\ensuremath{\gamma '[x \mapsto  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv_{2}}}}\endgroup }] \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv'}}}\endgroup } \in  {\mathcal{V}}\llbracket \tau _{2}/\Gamma \rrbracket }}} and the result holds.
	\end{subproof}
\item  {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }; \Gamma  \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\slambda}}}\endgroup } (x\mathrel{:}\tau _{1}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }).\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se'}}}\endgroup } \mathrel{:} (x:\tau _{1}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }) \xrightarrow {{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'}}}\endgroup }} \tau _{2} ; {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\varnothing }}}\endgroup }}}}
	\begin{subproof} 
		We know that 
		\begingroup\color{\colorMATH}\begin{gather*} 
			\inferrule*[lab={\textsc{ s-lam}}
		    ]{ \Gamma ,x\mathrel{:}\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }x\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se'}}}\endgroup } \mathrel{:} \tau _{2} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'}}}\endgroup }
		      }{
		      \Gamma  \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\slambda}}}\endgroup } (x\mathrel{:}\tau _{1}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }).\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se'}}}\endgroup } \mathrel{:} (x\mathrel{:}\tau _{1}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }) \overset {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'}}}\endgroup }\rightarrow  \tau _{2} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\varnothing }}}\endgroup }
		    }	
		\end{gather*}\endgroup
		We know that
		{{\color{\colorMATH}\ensuremath{\gamma  \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\slambda}}}\endgroup } (x\mathrel{:}\tau _{1}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }).\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se'}}}\endgroup } \Downarrow  \langle {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\slambda}}}\endgroup } (x\mathrel{:}\tau _{1}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }).\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se'}}}\endgroup }, \gamma \rangle }}}.
		We have to prove that 
		{{\color{\colorMATH}\ensuremath{\langle {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\slambda}}}\endgroup } (x\mathrel{:}\tau _{1}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }).\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se'}}}\endgroup }, \gamma \rangle  \in  {\mathcal{V}}\llbracket ((x:\tau _{1}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }) \xrightarrow {{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'}}}\endgroup }} \tau _{2})/\Gamma \rrbracket }}}.
		Suppose {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'}}}\endgroup } = {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS''}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'}}}\endgroup }x}}}, then 
		{{\color{\colorMATH}\ensuremath{((x:\tau _{1}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }) \xrightarrow {{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'}}}\endgroup }} \tau _{2})/\Gamma  = (x:\tau _{1}/\Gamma \mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }) \xrightarrow {{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'}}}\endgroup }x} (\tau _{2}/\Gamma )}}}.

		First, we have to prove that,
		{{\color{\colorMATH}\ensuremath{\langle {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\slambda}}}\endgroup } (x\mathrel{:}\tau _{1}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }).\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se'}}}\endgroup }, \gamma \rangle  \in  Atom\llbracket (x:\tau _{1}/\Gamma \mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }) \xrightarrow {{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'}}}\endgroup }x} (\tau _{2}/\Gamma )\rrbracket }}}, i.e. that
		 {{\color{\colorMATH}\ensuremath{\exists  \Gamma ', {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{0}}}}\endgroup }, dom({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS''}}}\endgroup }) \subseteq  dom(\Gamma ') \subseteq  dom({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{0}}}}\endgroup }), \forall  x_{i} \in  dom(\Gamma '), \varnothing ; \varnothing  \vdash  \gamma (x_{i}) : \tau '_i, \tau '_i <: \Gamma '(x_{i}) ; \varnothing , \Gamma '}}}, and {{\color{\colorMATH}\ensuremath{x: \tau _{1}; {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{0}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }x \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se'}}}\endgroup } \mathrel{:} \tau _{2} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS''}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'}}}\endgroup }x}}}.
		We prove this by choosing {{\color{\colorMATH}\ensuremath{\Gamma ' = \Gamma }}}, {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{0}}}}\endgroup } = {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }}}}, and {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS''}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'}}}\endgroup }x = {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'}}}\endgroup }}}}:
		 \begingroup\color{\colorMATH}\begin{gather*} 
			\inferrule*[lab=
			]{ \forall  x_{i} \in  dom(\Gamma ), \varnothing ; \varnothing  \vdash  \gamma (x_{i}) : \tau '_{i}, \tau '_{i} <: \Gamma (x_{i}) ; \varnothing 
			\\ \Gamma , x: \tau _{1}; {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss_{1}}}}\endgroup }x \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se'}}}\endgroup } \mathrel{:} \tau _{2} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS''}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'}}}\endgroup }x
			  }{
			  \Gamma ; {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \vdash  \langle {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\slambda}}}\endgroup } (x\mathrel{:}\tau _{1}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss_{1}}}}\endgroup }).\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se'}}}\endgroup }, \gamma \rangle  \mathrel{:} (x\mathrel{:} \tau _{1}/\Gamma '\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss_{1}}}}\endgroup }) \xrightarrow {{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'}}}\endgroup }x} \tau _{2}/\Gamma ' \mathrel{;} \varnothing 
			}
		\end{gather*}\endgroup

		Then we have prove that 
		{{\color{\colorMATH}\ensuremath{\forall  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv'}}}\endgroup } \in  {\mathcal{V}}\llbracket \tau _{1}/\Gamma \rrbracket , \gamma [x \mapsto  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv'}}}\endgroup }] \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se'}}}\endgroup } \in  {\mathcal{E}}\llbracket \tau _{2}/\Gamma \rrbracket }}}.
		By induction hypothesis on 
		{{\color{\colorMATH}\ensuremath{\Gamma ,x\mathrel{:}\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }x\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se'}}}\endgroup } \mathrel{:} \tau _{2} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'}}}\endgroup }}}}, we know that
		for any {{\color{\colorMATH}\ensuremath{\gamma ' \in  {\mathcal{G}}\llbracket \Gamma ,x:\tau _{1}\rrbracket }}}, {{\color{\colorMATH}\ensuremath{\gamma ' \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se'}}}\endgroup } \in  {\mathcal{E}}\llbracket \tau _{2}/\Gamma \rrbracket }}}.
		As {{\color{\colorMATH}\ensuremath{\gamma  \in  {\mathcal{G}}\llbracket \Gamma \rrbracket }}} and {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv'}}}\endgroup } \in  {\mathcal{V}}\llbracket \tau _{1}/\Gamma \rrbracket }}}, then
		{{\color{\colorMATH}\ensuremath{\gamma [x \mapsto  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv'}}}\endgroup }] \in  {\mathcal{G}}\llbracket \Gamma ,x:\tau _{1}\rrbracket }}}, so we pick 
		{{\color{\colorMATH}\ensuremath{\gamma ' = \gamma [x \mapsto  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv'}}}\endgroup }]}}} and the result holds.
		
	
	\end{subproof}
\end{enumerate}
Let us prove first (1).
We proceed by induction on {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }; \Gamma  \vdash 	{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe}}}\endgroup } : \tau  ; {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS}}}\endgroup }}}}.
\begin{enumerate}[ncases]\item  {{\color{\colorMATH}\ensuremath{\Gamma  \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorSYNTAX}\texttt{return}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \mathrel{:} [\varnothing /\wideparen{x}]\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup } + {\text{FS}}(\tau )}}}\endgroup }\lceil ^{\infty }}}}\endgroup }}}}
	\begin{subproof} 
		By {{\color{\colorMATH}\ensuremath{{\textsc{ return}}}}} we know that
		\begingroup\color{\colorMATH}\begin{gather*} 
		  \inferrule*[lab={\textsc{ return}}
		  ]{ \Gamma  \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \mathrel{:} \tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }
		  \\ \wideparen{x} = {\text{FV}}({\text{FS}}(\tau _{1}))
		    }{
		     \Gamma  \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorSYNTAX}\texttt{return}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \mathrel{:} [\varnothing /\wideparen{x}]\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup } + {\text{FS}}(\tau )}}}\endgroup }\lceil ^{\infty }}}}\endgroup }
		  }
		\end{gather*}\endgroup
		where {{\color{\colorMATH}\ensuremath{\tau  = [\varnothing /\wideparen{x}]\tau }}}, and {{\color{\colorMATH}\ensuremath{ {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS}}}\endgroup } = {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup } + {\text{FS}}(\tau _{1})}}}\endgroup }\lceil ^{\infty }}}}\endgroup }}}}.
		By induction hypotheses we know that
		{{\color{\colorMATH}\ensuremath{\gamma  \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \Downarrow  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv_{1}}}}\endgroup }}}}, and
		{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv_{1}}}}\endgroup } \in  {\mathcal{V}}\llbracket \tau _{1}/\Gamma \rrbracket }}}.

		Let us take some {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } \in  val_{*}}}}, if {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } \approx  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv_{1}}}}\endgroup }}}} then 
		{{\color{\colorMATH}\ensuremath{\llbracket {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{1}}}}\endgroup }\rrbracket _{\gamma } {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } = 1}}}, let us take another {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv'}}}\endgroup }}}}, if {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv'}}}\endgroup }\approx  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv_{1}}}}\endgroup }}}} then as {{\color{\colorMATH}\ensuremath{ {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv'}}}\endgroup } \in  val_{*}}}} it must be the case that {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv'}}}\endgroup } = {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }}}}, therefore if
		{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv'}}}\endgroup } \neq  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }}}} then {{\color{\colorMATH}\ensuremath{\llbracket {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{1}}}}\endgroup }\rrbracket _{\gamma } {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv'}}}\endgroup } = 0}}}. Finally {{\color{\colorMATH}\ensuremath{\Sigma  _{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } \in  val_{*}} \llbracket {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe}}}\endgroup }\rrbracket _{\gamma } {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } = 1}}} and the result holds.
	\end{subproof}
\item  {{\color{\colorMATH}\ensuremath{\Gamma  \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em} x: \tau _{1} \leftarrow  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{1}}}}\endgroup }\mathrel{;}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{2}}}}\endgroup } \mathrel{:} [\varnothing /x]\tau _{2} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{2}}}}\endgroup }}}}
	\begin{subproof} 
		By {{\color{\colorMATH}\ensuremath{{\textsc{ bind}}}}} we know that
		\begingroup\color{\colorMATH}\begin{gather*} 
		  \inferrule*[lab={\textsc{ bind}}
		  ]{ \Gamma  \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{1}}}}\endgroup } \mathrel{:} \tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{1}}}}\endgroup }
		  \\ \Gamma ,x\mathrel{:}\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{0}}}\endgroup }x   \hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{2}}}}\endgroup } \mathrel{:} \tau _{2} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{2}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{p}}}\endgroup }x
		    }{
		     \Gamma  \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em} x: \tau _{1} \leftarrow  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{1}}}}\endgroup }\mathrel{;}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{2}}}}\endgroup } \mathrel{:} [\varnothing /x]\tau _{2} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{2}}}}\endgroup }
		  }
		\end{gather*}\endgroup
		where {{\color{\colorMATH}\ensuremath{\tau  = [\varnothing /x]\tau _{2}}}}, and {{\color{\colorMATH}\ensuremath{ {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS}}}\endgroup } = {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{2}}}}\endgroup }}}}.
		By induction hypotheses we know that
		{{\color{\colorMATH}\ensuremath{\gamma  \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{1}}}}\endgroup } \in  {\mathcal{E}}\llbracket \tau _{1}\rrbracket }}}, therefore 
		{{\color{\colorMATH}\ensuremath{\Sigma _{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv'}}}\endgroup } \in  val_{*}(\tau /\gamma )}\llbracket {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{1}}}}\endgroup }\rrbracket _{\gamma }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv'}}}\endgroup } = 1}}}.

		Let us take some {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } \in  val_{*}(\tau /\gamma )}}}, if {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } \approx  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv_{1}}}}\endgroup }}}} then 
		{{\color{\colorMATH}\ensuremath{\llbracket {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{1}}}}\endgroup }\rrbracket _{\gamma } {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } = 1}}}, let us take another {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv'}}}\endgroup }}}}, if {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv'}}}\endgroup }\approx  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv_{1}}}}\endgroup }}}} then as {{\color{\colorMATH}\ensuremath{ {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv'}}}\endgroup } \in  val_{*}}}} it must be the case that {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv'}}}\endgroup } = {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }}}}, therefore if
		{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv'}}}\endgroup } \neq  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }}}} then {{\color{\colorMATH}\ensuremath{\llbracket {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{1}}}}\endgroup }\rrbracket _{\gamma } {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv'}}}\endgroup } = 0}}}. Finally {{\color{\colorMATH}\ensuremath{\Sigma  _{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } \in  val_{*}} \llbracket {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe}}}\endgroup }\rrbracket _{\gamma } {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } = 1}}} and the result holds.
	\end{subproof}
\end{enumerate}
\end{proof}

\begin{corollary}[Type Safety and Normalization of the Sensitivity Language]\;\\
  \label{lm:type-preservation-sensitivity}
  Let {{\color{\colorMATH}\ensuremath{\vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } : \tau  ; \varnothing }}}, then 
  {{\color{\colorMATH}\ensuremath{\vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \Downarrow  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }}}}, and {{\color{\colorMATH}\ensuremath{\vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }: \tau ';\varnothing }}}, where
  {{\color{\colorMATH}\ensuremath{\tau ' <: \tau }}}.
\end{corollary}
\begin{proof}
Direct consecuence of Prop~~\ref{lm:type-safety-FP}.
\end{proof}


Substitution:
\begingroup\color{\colorMATH}\begin{gather*}
	\begin{array}{rcl
	} [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{r}}}\endgroup } &{}={}& {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{r}}}\endgroup } 
	\cr  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]x &{}={}& {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }
	\cr  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup }) &{}={}& [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } + [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup }
	\cr  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \mathord{\cdotp } {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup }) &{}={}& [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \mathord{\cdotp } [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup }
	\cr  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \leq  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup }) &{}={}& [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \leq  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup }
	\cr  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\slambda}}}\endgroup } (x\mathrel{:}\tau _{1}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }).\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }) &{}={}& {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\slambda}}}\endgroup } (x\mathrel{:}[\varnothing /x]\tau _{1}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }).\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }
	\cr  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]({\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\plambda}}}\endgroup } (x\mathrel{:}\tau _{1}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }).\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe}}}\endgroup }) &{}={}& {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\plambda}}}\endgroup } (x\mathrel{:}[\varnothing /x]\tau _{1}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }).\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe}}}\endgroup }
	\cr  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup }) &{}={}& [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup }
	\cr  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]({{\color{\colorSYNTAX}\texttt{tt}}}) &{}={}& {{\color{\colorSYNTAX}\texttt{tt}}}
	\cr  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]({{\color{\colorSYNTAX}\texttt{inl}}}^{\tau _{2}}\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }) &{}={}& {{\color{\colorSYNTAX}\texttt{inl}}}^{[\varnothing /x]\tau _{2}}\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }
	\cr  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]({{\color{\colorSYNTAX}\texttt{inr}}}^{\tau _{1}}\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }) &{}={}& {{\color{\colorSYNTAX}\texttt{inr}}}^{[\varnothing /x]\tau _{1}}\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }
	\cr  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]({{\color{\colorSYNTAX}\texttt{case}}}\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{of}}}\hspace*{0.33em}\{ x\Rightarrow {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup }\} \hspace*{0.33em}\{ y\Rightarrow {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{3}}}}\endgroup }\} ) &{}={}& {{\color{\colorSYNTAX}\texttt{case}}}\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{of}}}\hspace*{0.33em}\{ x\Rightarrow [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup }\} \hspace*{0.33em}\{ y\Rightarrow [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{3}}}}\endgroup }\} 
	\cr  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x](\addProduct{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }}{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup }}) &{}={}& \addProduct{[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }}{[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup }}
	\cr  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]({{\color{\colorSYNTAX}\texttt{fst}}}\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }) &{}={}& {{\color{\colorSYNTAX}\texttt{fst}}}\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }
	\cr  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]({{\color{\colorSYNTAX}\texttt{snd}}}\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }) &{}={}& {{\color{\colorSYNTAX}\texttt{snd}}}\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }
	\cr  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x](\langle {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }, {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup }\rangle ) &{}={}& \langle [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }, [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup }\rangle 
	\cr  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]({{\color{\colorSYNTAX}\texttt{let}}}\hspace*{0.33em}x_{1},x_{2}={\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{in}}}\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup }) &{}={}& {{\color{\colorSYNTAX}\texttt{let}}}\hspace*{0.33em}x_{1},x_{2}=[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{in}}}\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup }
	\cr  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \mathrel{:: } \tau ) &{}={}& [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \mathrel{:: } [\varnothing /x]\tau 
	\cr  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]({\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorSYNTAX}\texttt{return}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }) &{}={}& {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorSYNTAX}\texttt{return}}}\endgroup }\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } 
	\cr  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x](z: \tau _{1} \leftarrow  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{1}}}}\endgroup }\mathrel{;}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{2}}}}\endgroup }) &{}={}& z: [\varnothing /x]\tau _{1} \leftarrow  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{1}}}}\endgroup }[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]\mathrel{;}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{2}}}}\endgroup } 
	\cr  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x](if\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }\hspace*{0.33em}\{ {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{2}}}}\endgroup }\} \hspace*{0.33em}\{ {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{3}}}}\endgroup }\} ) &{}={}& if\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }\hspace*{0.33em}\{ [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{2}}}}\endgroup }\} \hspace*{0.33em}\{ [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{3}}}}\endgroup }\} 
	\cr  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]({{\color{\colorSYNTAX}\texttt{case}}}\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{of}}}\hspace*{0.33em}\{ x\Rightarrow {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{2}}}}\endgroup }\} \hspace*{0.33em}\{ y\Rightarrow {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{3}}}}\endgroup }\} ) &{}={}& {{\color{\colorSYNTAX}\texttt{case}}}\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{of}}}\hspace*{0.33em}\{ x\Rightarrow [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{2}}}}\endgroup }\} \hspace*{0.33em}\{ y\Rightarrow [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{3}}}}\endgroup }\} 
	\cr  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]({\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{1}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{2}}}}\endgroup }) &{}={}& [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{1}}}}\endgroup }\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{2}}}}\endgroup }
	\end{array}
\end{gather*}\endgroup
\newcommand{\rop}{=}
\begin{lemma}[Type Preserving Substitution Lemma]
\label{lm:type-preservation-reviewerB}
Let {{\color{\colorMATH}\ensuremath{\tau _{1}}}} and {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }}}}, such that {{\color{\colorMATH}\ensuremath{ \varnothing ; \varnothing  \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } : \tau _{1} ; \varnothing }}}.	
% \begin{enumerate}\item  Let {{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1}; {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } : \tau _{2} ; {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup }}}}, then
% 	{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma ; [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \vdash  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } : \tau '_{2} ; {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'}}}\endgroup }}}}, where {{\color{\colorMATH}\ensuremath{\tau '_{2} \rop [\varnothing /x]\tau _{2}}}} and {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'}}}\endgroup } \rop [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup }}}}.
% \item  Let {{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1}; {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\vdash  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe}}}\endgroup } : \tau _{2} ; {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS}}}\endgroup }}}},  then
% 	{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma ; [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \vdash  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe}}}\endgroup } : \tau '_{2} ; {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS'}}}\endgroup }}}}, where {{\color{\colorMATH}\ensuremath{\tau '_{2} \rop [\varnothing /x]\tau _{2}}}} and {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS'}}}\endgroup } \rop [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS}}}\endgroup }}}}.
\begin{enumerate}\item  Let {{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1}; {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } : \tau _{2} ; {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup }}}}, then
	{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma ; [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \vdash  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } : [\varnothing /x]\tau _{2} ; [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup }}}}.
\item  Let {{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1}; {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\vdash  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe}}}\endgroup } : \tau _{2} ; {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS}}}\endgroup }}}},  then
	{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma ; [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \vdash  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe}}}\endgroup } : [\varnothing /x]\tau _{2} ; [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS}}}\endgroup }}}}.
\end{enumerate}	
\end{lemma}
\begin{proof}
We prove first (1).
We proceed by induction on type derivation {{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1}; {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } : \tau _{2} ; {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup }}}}.

\begin{enumerate}[ncases]\item  {{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{r}}}\endgroup } \mathrel{:} {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorSYNTAX}\texttt{{\ensuremath{{\mathbb{R}}}}}}}\endgroup } \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\varnothing }}}\endgroup }}}}
	\begin{subproof} 
		Trivial as {{\color{\colorMATH}\ensuremath{[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{r}}}\endgroup }= {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{r}}}\endgroup }}}}.
	\end{subproof}
\item  {{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }x\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}x \mathrel{:} \tau _{1} \mathrel{;} x }}}
	\begin{subproof} 
		We know that {{\color{\colorMATH}\ensuremath{[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]x = {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }}}}, and that 
		{{\color{\colorMATH}\ensuremath{\varnothing ; \varnothing  \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } : \tau '_{1} ; \varnothing }}}. We have to prove that
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma ; [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup } : \tau '_{1} ; \varnothing }}} (values are closed) where {{\color{\colorMATH}\ensuremath{\tau '_{1} \rop \tau _{1}}}}, and {{\color{\colorMATH}\ensuremath{\varnothing  \rop [\varnothing /x]x = \varnothing }}}, but we already know that and the result holds immediately.
	\end{subproof}
\item  {{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup } \mathrel{:} {\ensuremath{{\mathbb{R}}}} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup } {\ensuremath{+}} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }}}}
	\begin{subproof} 
		By definition of substitution {{\color{\colorMATH}\ensuremath{[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup }) = [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } + [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup }}}}.
		We apply induction hypotheses to 
		{{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \mathrel{:} {\ensuremath{{\mathbb{R}}}} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}}}, and 
		{{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup } \mathrel{:} {\ensuremath{{\mathbb{R}}}} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }}}}, so we know that
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma  \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \mathrel{:} {\ensuremath{{\mathbb{R}}}} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup }}}} where {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup } \rop [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}}}
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma  \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup } \mathrel{:} {\ensuremath{{\mathbb{R}}}} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup }}}} where {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup } \rop [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }}}}.
		Then by {{\color{\colorMATH}\ensuremath{{\textsc{ plus}}}}},
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma  \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } + [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup } \mathrel{:} {\ensuremath{{\mathbb{R}}}} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup } {\ensuremath{+}} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup }}}}, and as {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup } {\ensuremath{+}} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup } \rop [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup } {\ensuremath{+}} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }}}} the result holds.
	\end{subproof}
\item  {{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorSYNTAX}\texttt{{\ensuremath{\leq }}}}}\endgroup } {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup } \mathrel{:} {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorSYNTAX}\texttt{{\ensuremath{{\mathbb{B}}}}}}}\endgroup } \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorSYNTAX}\texttt{{\ensuremath{\infty (}}}}}\endgroup } {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup } {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorSYNTAX}\texttt{{\ensuremath{+}}}}}\endgroup } {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup } {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorSYNTAX}\texttt{{\ensuremath{)}}}}}\endgroup }}}}
	\begin{subproof} 
		By definition of substitution {{\color{\colorMATH}\ensuremath{[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \leq  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup }) = [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \leq  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup }}}}.
		We apply induction hypotheses to 
		{{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \mathrel{:} {\ensuremath{{\mathbb{R}}}} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}}}, and 
		{{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup } \mathrel{:} {\ensuremath{{\mathbb{R}}}} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }}}}, so we know that
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma  \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \mathrel{:} {\ensuremath{{\mathbb{R}}}} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup }}}} where {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup } \rop [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}}}
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma  \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup } \mathrel{:} {\ensuremath{{\mathbb{R}}}} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup }}}} where {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup } \rop [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }}}}.
		Then by {{\color{\colorMATH}\ensuremath{{\textsc{ leq}}}}},
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma  \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \leq  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup } \mathrel{:} {\ensuremath{{\mathbb{R}}}} \mathrel{;} \infty ({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup } {\ensuremath{+}} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup })}}}, and as {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup } {\ensuremath{+}} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup } \rop [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup } {\ensuremath{+}} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }}}} {{\color{\colorMATH}\ensuremath{ \infty ({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup } {\ensuremath{+}} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup }) \rop \infty ([\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup } {\ensuremath{+}} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup })}}} and the result holds.
	\end{subproof}
\item  {{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\slambda}}}\endgroup } (y\mathrel{:}\tau _{3}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }).\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se'}}}\endgroup } \mathrel{:} (y\mathrel{:}\tau _{3}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }) \oversetcustom{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'}}}\endgroup }x}\rightarrow   \tau _{4} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\varnothing }}}\endgroup }}}}
	\begin{subproof} 
		By definition of substitution {{\color{\colorMATH}\ensuremath{[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\slambda}}}\endgroup } (y\mathrel{:}\tau _{3}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }).\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se'}}}\endgroup }) = {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\slambda}}}\endgroup } (y\mathrel{:}[\varnothing /x]\tau _{3}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }).\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se'}}}\endgroup }}}}.
		Notice that {{\color{\colorMATH}\ensuremath{ [\varnothing /x]((y\mathrel{:}\tau _{3}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }) \oversetcustom{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'}}}\endgroup }x}\rightarrow   \tau _{4}) = (y\mathrel{:}[\varnothing /x]\tau _{3}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }) \oversetcustom{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}\rightarrow   [\varnothing /x]\tau _{4}}}}.
		We apply induction hypotheses to 
		{{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1}, y:\tau _{3} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se'}}}\endgroup } \mathrel{:} \tau _{4} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'}}}\endgroup }x}}}, to get 
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma , y:[\varnothing /x]\tau _{3} \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se'}}}\endgroup } \mathrel{:} [\varnothing /x]\tau '_{4} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup }}}}, where
		{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup } \rop [\varnothing /x]({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'}}}\endgroup }x) = {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}}} and {{\color{\colorMATH}\ensuremath{\tau '_{4} \rop [\varnothing /x]\tau _{4}}}}.

		Then by {{\color{\colorMATH}\ensuremath{{\textsc{ s-lam}}}}},
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma  \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\slambda}}}\endgroup } (y\mathrel{:}[\varnothing /x]\tau _{3}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }).\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se'}}}\endgroup } \mathrel{:} (y\mathrel{:}[\varnothing /x]\tau _{3}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }) \oversetcustom{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup }}\rightarrow   \tau '_{4} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\varnothing }}}\endgroup }}}}, but
		{{\color{\colorMATH}\ensuremath{(y\mathrel{:}[\varnothing /x]\tau _{3}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }) \oversetcustom{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup }}\rightarrow   \tau '_{4} \rop (y\mathrel{:}[\varnothing /x]\tau _{3}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }) \oversetcustom{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}\rightarrow   [\varnothing /x]\tau _{4}}}} and the result holds.

	\end{subproof}
\item  {{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\plambda}}}\endgroup } (x\mathrel{:}\tau _{3}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }).\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe'}}}\endgroup } \mathrel{:} (x\mathrel{:}\tau _{1}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }) \overset {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS'}}}\endgroup }\rightarrow  \tau _{4} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\varnothing }}}\endgroup }}}}
	\begin{subproof} 
		By definition of substitution {{\color{\colorMATH}\ensuremath{[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\slambda}}}\endgroup } (y\mathrel{:}\tau _{3}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }).\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe'}}}\endgroup }) = {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\slambda}}}\endgroup } (y\mathrel{:}[\varnothing /x]\tau _{3}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }).\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe'}}}\endgroup }}}}.
		Notice that {{\color{\colorMATH}\ensuremath{ [\varnothing /x]((y\mathrel{:}\tau _{3}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }) \oversetcustom{{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{1}}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{p'}}}\endgroup }x}\rightarrow   \tau _{4}) = (y\mathrel{:}[\varnothing /x]\tau _{3}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }) \oversetcustom{{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{1}}}}\endgroup }}\rightarrow   [\varnothing /x]\tau _{4}}}}.
		We apply induction hypotheses to 
		{{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1}, y:\tau _{3} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe'}}}\endgroup } \mathrel{:} \tau _{4} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{p'}}}\endgroup }x}}}, to get 
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma , y:[\varnothing /x]\tau _{3} \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe'}}}\endgroup } \mathrel{:} [\varnothing /x]\tau '_{4} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS'_{1}}}}\endgroup }}}}, where
		{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS'_{1}}}}\endgroup } \rop [\varnothing /x]({\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{1}}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{p'}}}\endgroup }x) = {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{1}}}}\endgroup }}}} and {{\color{\colorMATH}\ensuremath{\tau '_{4} \rop [\varnothing /x]\tau _{4}}}}.

		Then by {{\color{\colorMATH}\ensuremath{{\textsc{ p-lam}}}}},
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma  \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\slambda}}}\endgroup } (y\mathrel{:}[\varnothing /x]\tau _{3}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }).\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe'}}}\endgroup } \mathrel{:} (y\mathrel{:}[\varnothing /x]\tau _{3}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }) \oversetcustom{{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS'_{1}}}}\endgroup }}\rightarrow   \tau '_{4} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\varnothing }}}\endgroup }}}}, but
		{{\color{\colorMATH}\ensuremath{(y\mathrel{:}[\varnothing /x]\tau _{3}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }) \oversetcustom{{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS'_{1}}}}\endgroup }}\rightarrow   \tau '_{4} \rop (y\mathrel{:}[\varnothing /x]\tau _{3}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }) \oversetcustom{{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{1}}}}\endgroup }}\rightarrow   [\varnothing /x]\tau _{4}}}} and the result holds.
	\end{subproof}
\item  {{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup } \mathrel{:} [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }/y]\tau _{4} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss}}}\endgroup }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{3}}}}\endgroup }}}}
	\begin{subproof} 
		By definition of substitution {{\color{\colorMATH}\ensuremath{[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup }) = [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup }}}}.
		We apply induction hypotheses to 
		{{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \mathrel{:}  (y\mathrel{:}\tau _{3}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss_{1}}}}\endgroup }) \xrightarrow {{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{3}}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss_{2}}}}\endgroup }y } \tau _{4} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}}}, and 
		{{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup } \mathrel{:} \tau _{3} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }}}}, so we know that:
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma  \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \mathrel{:} (y\mathrel{:}\tau '_{3}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'_{1}}}}\endgroup }) \xrightarrow {{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{3}}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'_{2}}}}\endgroup }y } \tau '_{4} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup }}}} %(note that substitution does not change {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'}}}\endgroup }}}} annotations!) 
		where {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup } \rop [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}}}, and 
		{{\color{\colorMATH}\ensuremath{(y\mathrel{:}\tau '_{3}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'_{1}}}}\endgroup }) \xrightarrow {{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{3}}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'_{2}}}}\endgroup }y } \tau '_{4} \rop (y\mathrel{:}[\varnothing /x]\tau _{3}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss_{1}}}}\endgroup }) \xrightarrow {[\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{3}}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss_{2}}}}\endgroup }y } [\varnothing /x]\tau _{4}}}}, and that
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma  \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup } \mathrel{:} \tau ''_{3} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup }}}} where {{\color{\colorMATH}\ensuremath{\tau ''_{3} \rop [\varnothing /x]\tau _{3}}}} and {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup } \rop [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }}}}.
		But {{\color{\colorMATH}\ensuremath{[\varnothing /x]\tau _{3} \rop \tau '_{3}}}}, then {{\color{\colorMATH}\ensuremath{\tau ''_{3} \rop \tau '_{3}}}}.
		
		Then by {{\color{\colorMATH}\ensuremath{{\textsc{ s-app}}}}},
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma  \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup } \mathrel{:} [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup }/y]\tau '_{4} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'_{2}}}}\endgroup }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{3}}}}\endgroup }}}}, and as {{\color{\colorMATH}\ensuremath{\tau '_{4} \rop [\varnothing /x]\tau _{4} \Rightarrow  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup }/y]\tau '_{4} \rop [[\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }/y][\varnothing /x]\tau _{4} = [\varnothing /x][[\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }/y]\tau _{4}}}} and {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'_{2}}}}\endgroup }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{3}}}}\endgroup } \rop [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss_{2}}}}\endgroup }[\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup } + [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{3}}}}\endgroup }}}}.
		Also as {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \mathord{\cdotp } {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup } \leq  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss_{1}}}}\endgroup }}}}, we have to prove that {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{0}}}}\endgroup }\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup } \leq  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'_{1}}}}\endgroup }}}}. We know that {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss_{1}}}}\endgroup } \rop {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'_{1}}}}\endgroup }}}}, and as 
		{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{0}}}}\endgroup } \rop [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }}}} and {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup } \rop [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }}}}, then 
		{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{0}}}}\endgroup } \mathord{\cdotp } {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup } \rop	 [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \mathord{\cdotp } [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }}}}, then by transitivity
		{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{0}}}}\endgroup } \mathord{\cdotp } {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup } \leq  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'_{1}}}}\endgroup }}}} and the result holds.
	\end{subproof}
\item  {{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{tt}}} \mathrel{:} {{\color{\colorSYNTAX}\texttt{unit}}} \mathrel{;} \varnothing }}}
	\begin{subproof} 
		Trivial as {{\color{\colorMATH}\ensuremath{[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{{\color{\colorSYNTAX}\texttt{tt}}}= {{\color{\colorSYNTAX}\texttt{tt}}}}}}.
	\end{subproof}
\item  {{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{inl}}}^{\tau _{2}}\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \mathrel{:} \tau _{3} \mathrel{^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}\oplus ^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\varnothing }}}\endgroup }}} \tau _{4} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\varnothing }}}\endgroup }}}}
	\begin{subproof} 
		By definition of substitution {{\color{\colorMATH}\ensuremath{[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{{\color{\colorSYNTAX}\texttt{inl}}}^{\tau _{4}}\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } = [{{\color{\colorSYNTAX}\texttt{inl}}}^{[\varnothing /x]\tau _{4}}\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } }}}.
		We apply induction hypotheses to 
		{{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \mathrel{:} \tau _{3} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}}}, so we know that
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma  \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \mathrel{:} \tau '_{3} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup }}}} where {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup } \rop [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}}} and {{\color{\colorMATH}\ensuremath{\tau '_{3} \rop [\varnothing /x]\tau _{3}}}}.
		Then by {{\color{\colorMATH}\ensuremath{{\textsc{ inl}}}}},
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma  \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{inl}}}^{[\varnothing /x]\tau _{4}}\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \mathrel{:} \tau '_{3} \mathrel{^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup }}\oplus ^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\varnothing }}}\endgroup }}} [\varnothing /x]\tau _{4} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\varnothing }}}\endgroup }}}}, and as {{\color{\colorMATH}\ensuremath{\mathrel{^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup }}\oplus ^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\varnothing }}}\endgroup }}} \rop \mathrel{^{[\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup }}\oplus ^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\varnothing }}}\endgroup }}}}}} the result holds.
	\end{subproof}
\item  {{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{inr}}}^{\tau _{1}}\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \mathrel{:} \tau _{1} \mathrel{^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\varnothing }}}\endgroup }}\oplus ^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup }}} \tau _{2} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\varnothing }}}\endgroup }}}}
	\begin{subproof} 
		Analogous to {{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{inl}}}^{\tau _{2}}\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }}}} case.
	\end{subproof}
\item  {{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }  \hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{case}}}\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{of}}}\hspace*{0.33em}\{ x\Rightarrow {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup }\} \hspace*{0.33em}\{ y\Rightarrow {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{3}}}}\endgroup }\}  \mathrel{:} [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1 1}}}}\endgroup }/x]\tau _{4} \sqcup  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1 2}}}}\endgroup }/y]\tau _{3} \mathrel{;} (({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{s_{2}*\Sigma _{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{s_{2}\Sigma _{1 1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }) \sqcup  ({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{s_{3}*\Sigma _{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{s_{3}\Sigma _{1 2}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{3}}}}\endgroup }))}}}
	\begin{subproof} 
		By definition of substitution {{\color{\colorMATH}\ensuremath{[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]({{\color{\colorSYNTAX}\texttt{case}}}\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{of}}}\hspace*{0.33em}\{ z\Rightarrow {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup }\} \hspace*{0.33em}\{ y\Rightarrow {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{3}}}}\endgroup }\} ) = {{\color{\colorSYNTAX}\texttt{case}}}\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{of}}}\hspace*{0.33em}\{ z\Rightarrow [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup }\} \hspace*{0.33em}\{ y\Rightarrow [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{3}}}}\endgroup }\} }}}.
		We apply induction hypotheses to 
		{{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \mathrel{:} \tau _{1 1} \mathrel{^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1 1}}}}\endgroup }}\oplus ^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1 2}}}}\endgroup }}} \tau _{1 2} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}}}, 
		{{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1}, z\mathrel{:}\tau _{1 1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } + ({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\mathord{\cdotp }({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1 1}}}}\endgroup }))x \hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{ \vdash  e_{2}}}}\endgroup } \mathrel{:} \tau _{4} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss_{2}}}}\endgroup }z}}},
		{{\color{\colorMATH}\ensuremath{\Gamma ,x:\tau _{1}, y\mathrel{:}\tau _{1 2} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } + ({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\mathord{\cdotp }({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1 2}}}}\endgroup }))x \hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{ \vdash  e_{3}}}}\endgroup } \mathrel{:} \tau _{3} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{3}}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss_{3}}}}\endgroup }y}}} so we know that:
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma , x:\tau _{1} \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \mathrel{:} \tau '_{1 1} \mathrel{^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1 1}}}}\endgroup }}\oplus ^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1 2}}}}\endgroup }}} \tau '_{1 2} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup }}}}
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma , x:\tau _{1}, z\mathrel{:}\tau _{1 1} \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } + ([\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\mathord{\cdotp }([\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup } + [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1 1}}}}\endgroup }))x \hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{ \vdash }}}\endgroup } [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup } \mathrel{:} \tau '_{4} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'_{2}}}}\endgroup }z}}}, and
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma ,x:\tau _{1}, y\mathrel{:}\tau _{1 2} \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } + ([\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\mathord{\cdotp }([\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup } + [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1 2}}}}\endgroup }))x \hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{ \vdash }}}\endgroup } [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{3}}}}\endgroup } \mathrel{:} \tau '_{3} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{3}}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'_{3}}}}\endgroup }y}}},
		for {{\color{\colorMATH}\ensuremath{\tau '_{1 1} \rop	[\varnothing /x]\tau _{1 1}, {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1 1}}}}\endgroup } \rop [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1 1}}}}\endgroup }, {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1 2}}}}\endgroup } \rop [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1 2}}}}\endgroup }, {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup } \rop	[\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup },
		{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'_{2}}}}\endgroup }z \rop [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss_{2}}}}\endgroup }z, \tau '_{3} \rop [\varnothing /x]\tau _{3}}}}, and  {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{3}}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'_{3}}}}\endgroup }y \rop [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{3}}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss_{3}}}}\endgroup }y}}}.
		
		Then by {{\color{\colorMATH}\ensuremath{{\textsc{ s-case}}}}},
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }  \hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{case}}}\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{of}}}\hspace*{0.33em}\{ x\Rightarrow [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup }\} \hspace*{0.33em}\{ y\Rightarrow [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{3}}}}\endgroup }\}  \mathrel{:} [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1 1}}}}\endgroup }/x]\tau '_{4} \sqcup  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1 2}}}}\endgroup }/y]\tau '_{3} \mathrel{;} (({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{s'_{2}*\Sigma '_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{s'_{2}\Sigma '_{1 1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup }) \sqcup  ({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{s'_{3}*\Sigma '_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{s'_{3}\Sigma '_{1 2}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{3}}}}\endgroup }))}}}.
		We know that 
		{{\color{\colorMATH}\ensuremath{[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1 1}}}}\endgroup }/x]\tau '_{4} \rop [[\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup } + [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1 1}}}}\endgroup }/x][\varnothing /x]\tau '_{4} = [\varnothing /x][{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1 1}}}}\endgroup }/x]\tau '_{4}}}}, and
		{{\color{\colorMATH}\ensuremath{[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1 2}}}}\endgroup }/x]\tau '_{3} \rop [[\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup } + [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1 2}}}}\endgroup }/x][\varnothing /x]\tau '_{3} = [\varnothing /x][{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1 2}}}}\endgroup }/x]\tau '_{3}}}}, therefore 
		{{\color{\colorMATH}\ensuremath{[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1 1}}}}\endgroup }/x]\tau '_{4} \sqcup  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1 2}}}}\endgroup }/y]\tau '_{3} \rop [\varnothing /x][{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1 1}}}}\endgroup }/x]\tau '_{4} \sqcup  [\varnothing /x][{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1 2}}}}\endgroup }/y]\tau '_{3}}}}.
		Also {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{s'_{2}*\Sigma '_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{s'_{2}\Sigma '_{1 1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup }) \rop {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{s_{2}*[\varnothing /x]\Sigma _{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{s_{2}[\varnothing /x]\Sigma _{1 1}}}}\endgroup } + [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup })}}}, and {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{s'_{3}*\Sigma '_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{s'_{3}\Sigma '_{1 2}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{3}}}}\endgroup }) \rop {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{s_{3}*[\varnothing /x]\Sigma _{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{s_{3}[\varnothing /x]\Sigma _{1 2}}}}\endgroup } + [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{3}}}}\endgroup })}}} and the result holds.
	\end{subproof}
\item  {{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }  \hspace*{0.33em} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{ \vdash  }}}\endgroup }\hspace*{0.33em} \hspace*{0.33em}\addProduct{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }}{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup }} \mathrel{:} \tau _{3} \mathrel{^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}\&^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }}} \tau _{4} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\varnothing }}}\endgroup }}}}
	\begin{subproof} 
		By definition of substitution {{\color{\colorMATH}\ensuremath{[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]\addProduct{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }}{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup }} = \addProduct{[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }}{[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup }}}}}.
		We apply induction hypotheses to 
		{{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \mathrel{:} \tau _{3} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}}}, and 
		{{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup } \mathrel{:} \tau _{4} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }}}}, so we know that
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma  \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \mathrel{:} \tau '_{3} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup }}}} where {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup } \rop [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}}} and {{\color{\colorMATH}\ensuremath{\tau '_{3} \rop [\varnothing /x]\tau _{3}}}}
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma  \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup } \mathrel{:} \tau '_{4} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup }}}} where {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup } \rop [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }}}} and 
		{{\color{\colorMATH}\ensuremath{\tau '_{4} \rop [\varnothing /x]\tau _{4}}}}.
		Then by {{\color{\colorMATH}\ensuremath{{\textsc{ pair}}}}},
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma  \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}\addProduct{[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }}{[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup }} \mathrel{:} \tau '_{3} \mathrel{^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup }}\&^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup }}} \tau '_{4} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\varnothing }}}\endgroup }}}}, and as {{\color{\colorMATH}\ensuremath{\tau '_{3} \mathrel{^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup }}\&^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup }}} \tau '_{4} \rop [\varnothing /x]\tau '_{3} \mathrel{^{[\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup }}\&^{[\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup }}} [\varnothing /x]\tau '_{4}}}} the result holds.
	\end{subproof}
\item  {{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }  \hspace*{0.33em} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{ \vdash  }}}\endgroup }\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{fst}}}\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \mathrel{:} \tau _{3} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{3}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}}}
	\begin{subproof} 
		By definition of substitution {{\color{\colorMATH}\ensuremath{[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{{\color{\colorSYNTAX}\texttt{fst}}}\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } = {{\color{\colorSYNTAX}\texttt{fst}}}\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } }}}.
		We apply induction hypotheses to 
		{{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \mathrel{:} \tau _{3} \mathrel{^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}\&^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }}} \tau _{4} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{3}}}}\endgroup }}}}, so we know that
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma  \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \mathrel{:} \tau '_{3} \mathrel{^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup }}\&^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup }}} \tau '_{4} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{3}}}}\endgroup }}}} where {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{i}}}}\endgroup } \rop [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{i}}}}\endgroup }}}}, {{\color{\colorMATH}\ensuremath{\tau '_{3} \rop [\varnothing /x]\tau _{3}}}}, and {{\color{\colorMATH}\ensuremath{\tau '_{4} \rop [\varnothing /x]\tau _{4}}}}.
		Then by {{\color{\colorMATH}\ensuremath{{\textsc{ proj1}}}}},
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma  \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{fst}}}\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \mathrel{:} \tau '_{3} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{3}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup }}}}, and as {{\color{\colorMATH}\ensuremath{ {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{3}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup } \rop  [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{3}}}}\endgroup } + [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup }}}} the result holds.
	\end{subproof}
\item  {{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }  \hspace*{0.33em} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{ \vdash  }}}\endgroup }\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{snd}}}\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup } \mathrel{:} \tau _{2} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }}}}
	\begin{subproof} 
		Analogous to {{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{fst}}}\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se}}}\endgroup }}}} case.
	\end{subproof}
\item  {{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }  \hspace*{0.33em} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{ \vdash  }}}\endgroup }\hspace*{0.33em}\langle {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }, {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup }\rangle  \mathrel{:} \tau _{1} \mathrel{^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}\otimes ^{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }}} \tau _{2} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{ \varnothing  }}}\endgroup }}}}
	\begin{subproof} 
		Analogous to {{\color{\colorMATH}\ensuremath{\addProduct{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }}{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup }}}}} case.
	\end{subproof}
\item  {{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }  \hspace*{0.33em} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{ \vdash  }}}\endgroup }\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{let}}}\hspace*{0.33em}x_{1},x_{2}={\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{in}}}\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup } \mathrel{:} [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1 1}}}}\endgroup }/x_{1}][{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1 2}}}}\endgroup }/x_{2}]\tau _{2} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss_{1}}}}\endgroup }({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1 1}}}}\endgroup })+ {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss_{2}}}}\endgroup }({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1 2}}}}\endgroup }) + {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }}}}
	\begin{subproof} 
		Similar to {{\color{\colorMATH}\ensuremath{{{\color{\colorSYNTAX}\texttt{case}}}}}} case.
	\end{subproof}
\item  {{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \vdash  {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorSYNTAX}\texttt{{\ensuremath{ {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \mathrel{:: } {{\color{\colorMATH}\ensuremath{\tau _{3}}}} }}}}}\endgroup })}}}\endgroup } \mathrel{:} {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{\tau _{3}}}}\endgroup } \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}}}
	\begin{subproof} 
		By definition of substitution {{\color{\colorMATH}\ensuremath{[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } :: \tau _{3}) = [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } ::[\varnothing /x]\tau _{3} }}}.
		We apply induction hypotheses to 
		{{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \mathrel{:} \tau _{4} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}}}, so we know that
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma  \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \mathrel{:} \tau '_{4} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup }}}} where {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup } \rop [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}}} and {{\color{\colorMATH}\ensuremath{\tau '_{4} \rop [\varnothing /x]\tau _{4}}}}.
		We also know that if {{\color{\colorMATH}\ensuremath{\tau '_{4} \rop [\varnothing /x]\tau _{4}}}}, {{\color{\colorMATH}\ensuremath{\tau _{4} <: \tau _{3}}}} then {{\color{\colorMATH}\ensuremath{[\varnothing /x]\tau _{4} <: [\varnothing /x]\tau _{3}}}}, and thus {{\color{\colorMATH}\ensuremath{\tau '_{4} <: [\varnothing /x]\tau _{3}}}}
		Then by {{\color{\colorMATH}\ensuremath{{\textsc{ asc}}}}},
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma  \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } ::[\varnothing /x]\tau _{3} \mathrel{:} [\varnothing /x]\tau _{3} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup }}}}, and the result holds.
	\end{subproof}
\end{enumerate}

We prove now (2).
We proceed by induction on type derivation {{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1}; {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\vdash  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe}}}\endgroup } : \tau _{2} ; {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS}}}\endgroup }}}}.

\begin{enumerate}[ncases]\item  {{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorSYNTAX}\texttt{return}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \mathrel{:} [\varnothing /\wideparen{x}]\tau _{3} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup } + {\text{FS}}(\tau _{3})}}}\endgroup }\lceil ^{\infty }}}}\endgroup }}}}
	\begin{subproof} 
		By definition of substitution {{\color{\colorMATH}\ensuremath{[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorSYNTAX}\texttt{return}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } = {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorSYNTAX}\texttt{return}}}\endgroup }\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } }}}.
		We apply induction hypotheses to 
		{{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{3} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \mathrel{:} \tau _{3} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}}}, so we know that
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma  \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \mathrel{:} \tau '_{3} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup }}}} where {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup } \rop [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}}}, {{\color{\colorMATH}\ensuremath{\tau '_{3} \rop [\varnothing /x]\tau _{3}}}}.

		Let {{\color{\colorMATH}\ensuremath{\wideparen{y} = {\text{FV}}({\text{FS}}(\tau '_{3}))}}}.
		Note that {{\color{\colorMATH}\ensuremath{[\varnothing /x]{\text{FS}}(\tau '_{3}) = {\text{FS}}([\varnothing /x]\tau '_{3})}}}, and that {{\color{\colorMATH}\ensuremath{[\varnothing /\wideparen{y}][\varnothing /x]\tau '_{3} = [\varnothing /x][\varnothing /\wideparen{y}]\tau '_{3}}}}.
		Also {{\color{\colorMATH}\ensuremath{[\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup } + [\varnothing /x]{\text{FS}}(\tau _{3}) = [\varnothing /x]({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup } + {\text{FS}}(\tau _{3}))}}}, and
	    {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil }}}\endgroup }[\varnothing /x]({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup } + {\text{FS}}(\tau _{3})){\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\lceil ^{\infty }}}}\endgroup } = [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup } + {\text{FS}}(\tau _{3})}}}\endgroup }\lceil ^{\infty }}}}\endgroup }}}}.
		Then by {{\color{\colorMATH}\ensuremath{{\textsc{ return}}}}},
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma  \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorSYNTAX}\texttt{return}}}\endgroup }\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \mathrel{:} [\varnothing /\wideparen{y}]\tau '_{3} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup } + {\text{FS}}(\tau '_{3})}}}\endgroup }\lceil ^{\infty }}}}\endgroup }}}}.
		We know that
		{{\color{\colorMATH}\ensuremath{[\varnothing /\wideparen{y}]\tau '_{3} = [\varnothing /{\text{FV}}({\text{FS}}(\tau '_{3}))]\tau '_{3}}}}, but {{\color{\colorMATH}\ensuremath{\tau '_{3} \rop [\varnothing /x]\tau _{3}}}},
		and {{\color{\colorMATH}\ensuremath{[\varnothing /x]{\text{FV}}({\text{FS}}(\tau _{3})) = {\text{FV}}({\text{FS}}([\varnothing /x]\tau _{3}))}}}, then
		{{\color{\colorMATH}\ensuremath{[\varnothing /{\text{FV}}({\text{FS}}(\tau '_{3}))]\tau '_{3} \rop [\varnothing /x]([\varnothing /{\text{FV}}({\text{FS}}(\tau _{3}))]\tau _{3})}}}.
		Also {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup } + {\text{FS}}(\tau '_{3})}}}\endgroup }\lceil ^{\infty }}}}\endgroup } \rop {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{[\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup } + {\text{FS}}([\varnothing /x]\tau _{3})}}}\endgroup }\lceil ^{\infty }}}}\endgroup } = [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup } + {\text{FS}}(\tau _{3})}}}\endgroup }\lceil ^{\infty }}}}\endgroup }}}} and the result holds.
	\end{subproof}
\item  {{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em} z: \tau _{3} \leftarrow  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{1}}}}\endgroup }\mathrel{;}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{2}}}}\endgroup } \mathrel{:} [\varnothing /z]\tau _{4} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{2}}}}\endgroup }}}}
	\begin{subproof} 
		By definition of substitution {{\color{\colorMATH}\ensuremath{[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x](z: \tau _{3} \leftarrow  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{1}}}}\endgroup }\mathrel{;}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{2}}}}\endgroup } ) = z: [\varnothing /x]\tau _{3} \leftarrow  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{1}}}}\endgroup }\mathrel{;}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{2}}}}\endgroup }}}}.
		We apply induction hypotheses to 
		{{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{1}}}}\endgroup } \mathrel{:} \tau _{3} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{1}}}}\endgroup }}}}, and 
		{{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} z: \tau _{3} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{0}}}\endgroup }z\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{2}}}}\endgroup } \mathrel{:} \tau _{4} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{2}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{p}}}\endgroup }z}}}, so we know that:
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma  \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{1}}}}\endgroup } \mathrel{:} \tau '_{3} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS'_{1}}}}\endgroup }}}} %(note that substitution does not change {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'}}}\endgroup }}}} annotations!) 
		where {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS'_{1}}}}\endgroup } \rop [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{1}}}}\endgroup }}}}, and 
		{{\color{\colorMATH}\ensuremath{\tau '_{3} \rop [\varnothing /x]\tau _{3}}}}, and that
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma , z: \tau _{3}\mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{0}}}\endgroup }z\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{2}}}}\endgroup } \mathrel{:} \tau '_{4} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS'_{2}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{p'}}}\endgroup }z}}} 
		where {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS'_{2}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{p'}}}\endgroup }z \rop [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{2}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{p}}}\endgroup }z}}} and {{\color{\colorMATH}\ensuremath{\tau '_{4} \rop [\varnothing /x]\tau _{4}}}}.
		
		Then by {{\color{\colorMATH}\ensuremath{{\textsc{ bind}}}}},
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma  \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em} z: [\varnothing /x]\tau _{3} \leftarrow  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{1}}}}\endgroup }\mathrel{;}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{2}}}}\endgroup } \mathrel{:} [\varnothing /z]\tau '_{4} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS'_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS'_{2}}}}\endgroup }}}}, 
		and as {{\color{\colorMATH}\ensuremath{\tau '_{4} \rop [\varnothing /x]\tau _{4} \Rightarrow  [[\varnothing /z]\tau '_{4} \rop [\varnothing /z][\varnothing /x]\tau '_{4} = [\varnothing /x][\varnothing /z]\tau _{4}}}} and {{\color{\colorMATH}\ensuremath{ {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS'_{1}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS'_{2}}}}\endgroup } \rop [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{1}}}}\endgroup } + [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{2}}}}\endgroup }}}} the result holds.
		
	\end{subproof}
\item  {{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em} if\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }\hspace*{0.33em}\{ {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{2}}}}\endgroup }\} \hspace*{0.33em}\{ {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{3}}}}\endgroup }\}  \mathrel{:} \tau _{3} \mathrel{;}  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}}}\endgroup }\lceil ^{\infty }}}}\endgroup } + ({\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{2}}}}\endgroup } \sqcup  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{3}}}}\endgroup })}}}
	\begin{subproof} 
		By definition of substitution {{\color{\colorMATH}\ensuremath{[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x](if\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }\hspace*{0.33em}\{ {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{2}}}}\endgroup }\} \hspace*{0.33em}\{ {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{3}}}}\endgroup }\} ) = z: [\varnothing /x]\tau _{3} \leftarrow  if\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }\hspace*{0.33em}\{ [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{2}}}}\endgroup }\} \hspace*{0.33em}\{ [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{3}}}}\endgroup }\} }}}.
		We apply induction hypotheses to 
		{{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \mathrel{:} {\mathbb{B}} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}}},
		{{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{2}}}}\endgroup } \mathrel{:} \tau _{3} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{2}}}}\endgroup }}}}, and
		{{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{3}}}}\endgroup } \mathrel{:} \tau _{3} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{3}}}}\endgroup }}}}
		so we know that:
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma  \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \mathrel{:} {\mathbb{B}} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup }}}},
		where {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup } \rop [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}}}, and 
		{{\color{\colorMATH}\ensuremath{\tau '_{3} \rop [\varnothing /x]\tau _{3}}}},
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma  \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{2}}}}\endgroup } \mathrel{:} \tau '_{3} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS'_{2}}}}\endgroup }}}},
		where {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS'_{2}}}}\endgroup } \rop [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{2}}}}\endgroup }}}}, and 
		{{\color{\colorMATH}\ensuremath{\tau '_{3} \rop [\varnothing /x]\tau _{3}}}}, and that
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{3}}}}\endgroup } \mathrel{:} \tau '_{4} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS'_{3}}}}\endgroup }}}} 
		where {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS'_{3}}}}\endgroup } \rop [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{3}}}}\endgroup }}}} and {{\color{\colorMATH}\ensuremath{\tau '_{4} \rop [\varnothing /x]\tau _{3}}}}.
		Note that {{\color{\colorMATH}\ensuremath{\tau '_{3} = \tau '_{4}}}}.

		
		Then by {{\color{\colorMATH}\ensuremath{{\textsc{ if}}}}},
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma  \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em} if\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }\hspace*{0.33em}\{ [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{2}}}}\endgroup }\} \hspace*{0.33em}\{ [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{3}}}}\endgroup } \mathrel{:} \tau '_{3} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup }}}}\endgroup }\lceil ^{\infty }}}}\endgroup } + ({\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS'_{2}}}}\endgroup } \sqcup  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS'_{3}}}}\endgroup })}}}.
		Note that 
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]({\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}}}\endgroup }\lceil ^{\infty }}}}\endgroup } + ({\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{2}}}}\endgroup } \sqcup  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{3}}}}\endgroup })) = {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{[\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}}}\endgroup }\lceil ^{\infty }}}}\endgroup } + ([\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{2}}}}\endgroup } \sqcup  [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{3}}}}\endgroup }) = }}} 
		Note that as {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup } \rop [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}}} then {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup }}}}\endgroup }\lceil ^{\infty }}}}\endgroup } \rop {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{[\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}}}\endgroup }\lceil ^{\infty }}}}\endgroup }}}}.
		Also as {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS'_{2}}}}\endgroup } \rop [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{2}}}}\endgroup }}}} and {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS'_{3}}}}\endgroup } \rop [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{3}}}}\endgroup }}}} then
		{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS'_{2}}}}\endgroup } \sqcup  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS'_{3}}}}\endgroup } \rop	 [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{2}}}}\endgroup } \sqcup  [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{3}}}}\endgroup } = [\varnothing /x]({\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS'_{2}}}}\endgroup } \sqcup  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS'_{3}}}}\endgroup })}}}.
		Then {{\color{\colorMATH}\ensuremath{ {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup }}}}\endgroup }\lceil ^{\infty }}}}\endgroup } + ({\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS'_{2}}}}\endgroup } \sqcup  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS'_{3}}}}\endgroup }) \rop [\varnothing /x]({\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}}}\endgroup }\lceil ^{\infty }}}}\endgroup } + ({\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{2}}}}\endgroup } \sqcup  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{3}}}}\endgroup }))}}} and the result holds.
		
	\end{subproof}
\item  {{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em} {{\color{\colorSYNTAX}\texttt{case}}}\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup }\hspace*{0.33em}{{\color{\colorSYNTAX}\texttt{of}}}\hspace*{0.33em}\{ x\Rightarrow {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{2}}}}\endgroup }\} \hspace*{0.33em}\{ y\Rightarrow {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{3}}}}\endgroup }\}  \mathrel{:} [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1 1}}}}\endgroup }/x]\tau _{4} \sqcup  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1 2}}}}\endgroup }/y]\tau _{3} \mathrel{;}  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \times  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}}}\endgroup }\lceil ^{\infty }}}}\endgroup } + (( {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1 1}}}}\endgroup }\lceil ^{p_{2}}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{2}}}}\endgroup }) \sqcup  ( {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1 2}}}}\endgroup }\lceil ^{p_{3}}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{3}}}}\endgroup }))}}}
	\begin{subproof} 
		Analogous to {{\color{\colorMATH}\ensuremath{{\textsc{ s-case}}}}} case.
	\end{subproof}
\item  {{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{1}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{2}}}}\endgroup } \mathrel{:} [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }/y]\tau _{4} \mathrel{;}  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \times  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}}}\endgroup }\lceil ^{\infty }}}}\endgroup } +  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \times  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }}}}\endgroup }\lceil ^{p}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{3}}}}\endgroup }}}}
	\begin{subproof} 
		By definition of substitution {{\color{\colorMATH}\ensuremath{[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]({\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{1}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{2}}}}\endgroup }) = [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{1}}}}\endgroup }\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{2}}}}\endgroup }}}}.
		We apply induction hypotheses to 
		{{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \mathrel{:}  (y\mathrel{:}\tau _{3}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss_{1}}}}\endgroup }) \xrightarrow {{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{3}}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{p}}}\endgroup }y } \tau _{4} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}}}, and 
		{{\color{\colorMATH}\ensuremath{\Gamma , x:\tau _{1} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup } \mathrel{:} \tau _{3} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }}}}, so we know that:
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma  \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{1}}}}\endgroup } \mathrel{:} (y\mathrel{:}\tau '_{3}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'_{1}}}}\endgroup }) \xrightarrow {{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS'_{3}}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{p'}}}\endgroup }y } \tau '_{4} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup }}}} %(note that substitution does not change {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'}}}\endgroup }}}} annotations!) 
		where {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup } \rop [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}}}, and 
		{{\color{\colorMATH}\ensuremath{(y\mathrel{:}\tau '_{3}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss'_{1}}}}\endgroup }) \xrightarrow {{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS'_{3}}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{p'}}}\endgroup }y } \tau '_{4} \rop (y\mathrel{:}[\varnothing /x]\tau _{3}\mathord{\cdotp }{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sss_{1}}}}\endgroup }) \xrightarrow {[\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{3}}}}\endgroup }+{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{p}}}\endgroup }y } [\varnothing /x]\tau _{4}}}}, and that
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma  \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\se_{2}}}}\endgroup } \mathrel{:} \tau ''_{3} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup }}}} where {{\color{\colorMATH}\ensuremath{\tau ''_{3} \rop [\varnothing /x]\tau _{3}}}} and {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup } \rop [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }}}}.
		But {{\color{\colorMATH}\ensuremath{[\varnothing /x]\tau _{3} \rop \tau '_{3}}}}, then {{\color{\colorMATH}\ensuremath{\tau ''_{3} \rop \tau '_{3}}}}.
		
		Then by {{\color{\colorMATH}\ensuremath{{\textsc{ p-app}}}}},
		{{\color{\colorMATH}\ensuremath{[\varnothing /x]\Gamma  \mathrel{;} [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup }\hspace*{0.33em}{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\vdash }}}\endgroup }\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{1}}}}\endgroup }\hspace*{0.33em}[{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sv}}}\endgroup }/x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pe_{2}}}}\endgroup } \mathrel{:} [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup }/y]\tau '_{4} \mathrel{;} {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{[\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \times  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup }}}}\endgroup }\lceil ^{\infty }}}}\endgroup } +  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{[\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \times  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup }}}}\endgroup }\lceil ^{p'}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS'_{3}}}}\endgroup }}}}. 
		Note that {{\color{\colorMATH}\ensuremath{\tau '_{4} \rop [\varnothing /x]\tau _{4} \Rightarrow  [{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup }/y]\tau '_{4} \rop [[\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }/y][\varnothing /x]\tau _{4} = [\varnothing /x][[\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }/y]\tau _{4}}}}.
		Also as {{\color{\colorMATH}\ensuremath{[\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \times  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup } \rop	 [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \times  [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup } = [\varnothing /x]({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \times  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup })}}}, then {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{[\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \times  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup }}}}\endgroup }\lceil ^{\infty }}}}\endgroup } \rop {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{[\varnothing /x]({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \times  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup })}}}\endgroup }\lceil ^{\infty }}}}\endgroup } = [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \times  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{1}}}}\endgroup }}}}\endgroup }\lceil ^{\infty }}}}\endgroup }}}}. Similarly, 
		{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{[\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \times  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup }}}}\endgroup }\lceil ^{\infty }}}}\endgroup } \rop {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{[\varnothing /x]({\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \times  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup })}}}\endgroup }\lceil ^{\infty }}}}\endgroup } = [\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \times  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{2}}}}\endgroup }}}}\endgroup }\lceil ^{\infty }}}}\endgroup }}}}.
		Therefore {{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{[\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \times  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup }}}}\endgroup }\lceil ^{\infty }}}}\endgroup } +  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{[\varnothing /x]{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \times  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup }}}}\endgroup }\lceil ^{p'}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS'_{3}}}}\endgroup } \rop [\varnothing /x]({\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \times  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{1}}}}\endgroup }}}}\endgroup }\lceil ^{\infty }}}}\endgroup } +  {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\rceil {\begingroup\renewcommand\colorMATH{\colorMATHA}\renewcommand\colorSYNTAX{\colorSYNTAXA}{{\color{\colorMATH}\ensuremath{{\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS_{0}}}}\endgroup } \times  {\begingroup\renewcommand\colorMATH{\colorMATHB}\renewcommand\colorSYNTAX{\colorSYNTAXB}{{\color{\colorMATH}\ensuremath{\sS'_{2}}}}\endgroup }}}}\endgroup }\lceil ^{p'}}}}\endgroup } + {\begingroup\renewcommand\colorMATH{\colorMATHC}\renewcommand\colorSYNTAX{\colorSYNTAXC}{{\color{\colorMATH}\ensuremath{\pS_{3}}}}\endgroup })}}} and the result holds.
	\end{subproof}
\end{enumerate}

\end{proof}
% Let us analize the case t = (\lambda x. (\lambda y. x + y)) 1 2.
% We'll show that if \vdash  t: T;\varnothing , and t \Downarrow  v then \vdash  v: T;\varnothing .


% Let 

%     }{     }{
%     x:{\mathbb{R}}, y:{\mathbb{R}}; \infty x+\infty y \vdash  x : {\mathbb{R}}; x     x:{\mathbb{R}}, y:{\mathbb{R}}; \infty x+\infty y \vdash  y : {\mathbb{R}}; y
%     }{
%              x:{\mathbb{R}}, y:{\mathbb{R}}; \infty x+\infty y \vdash  x + y : {\mathbb{R}}; x + y
%         }{
%           x:{\mathbb{R}}; \infty x \vdash  (\lambda y. x + y) : (y: {\mathbb{R}}) --x+y\rightarrow  {\mathbb{R}}; 0x
% D_{1} =   }{
%       \varnothing ; \varnothing  \vdash  (\lambda x. (\lambda y. x + y)) : (x: {\mathbb{R}}) --0x\rightarrow  (y: {\mathbb{R}}) --x+y\rightarrow  {\mathbb{R}}; \varnothing 


% As, \varnothing ;\varnothing \vdash 1:{\mathbb{R}}; \varnothing , and [\varnothing /x]((y: {\mathbb{R}}) --x+y\rightarrow  {\mathbb{R}}) = (y: {\mathbb{R}}) --y\rightarrow  {\mathbb{R}}, then:

%                             }{ 
%                 D_{1}          \varnothing ;\varnothing \vdash 1:{\mathbb{R}}; \varnothing   
% D_{2} = }{
%       \varnothing ; \varnothing  \vdash  (\lambda x. (\lambda y. x + y)) 1 : (y: {\mathbb{R}}) --y\rightarrow  {\mathbb{R}}; \varnothing 


%                         }{
%                D_{2}       \varnothing ;\varnothing \vdash 2:{\mathbb{R}}; \varnothing      
% D_{3} = }{
%        \varnothing ; \varnothing  \vdash  ((\lambda x. (\lambda y. x + y)) 1) 2 : {\mathbb{R}}; \varnothing 


% Let us start focusing on the reduction of \langle \lambda x. (\lambda y. x + y), \varnothing \rangle  1

%            \varnothing  \vdash  (\lambda x. (\lambda y. x + y)) \Downarrow  \langle \lambda x. (\lambda y. x + y), \varnothing \rangle     
%            \varnothing  \vdash  1 \Downarrow  1
%        x \mapsto  1 \vdash  (\lambda y. x + y) \Downarrow  \langle \lambda y. x + y, x \mapsto  1\rangle 
% R_{1} =  }{
%      \varnothing  \vdash  \langle \lambda x. (\lambda y. x + y), \varnothing \rangle  1 \Downarrow  \langle \lambda y. x + y, x \mapsto  1\rangle 


% At this point type rule for closures removes x from scope at the end:
%                ...
%    }{
%    x:{\mathbb{R}}, y:{\mathbb{R}}; \infty x+\infty y \vdash  x + y : {\mathbb{R}}; x + y
% }{
% \varnothing ;\varnothing  \vdash  \langle \lambda y. x + y, x \mapsto  1\rangle  : (y: {\mathbb{R}}) --y\rightarrow  {\mathbb{R}}



% Therefore the whole term reduces as follows:

% R_{1}
% \varnothing  \vdash  2 \Downarrow  2
% x \mapsto  1, y \mapsto  2 \vdash  x + y \Downarrow  3
% }{
% \varnothing  \vdash  ((\lambda x. (\lambda y. x + y)) 1) 2  \Downarrow  3

% And \varnothing ;\varnothing  \vdash  3 : {\mathbb{R}}; \varnothing  so the type is preserved after reduction.
% (\lambda x: {\mathbb{R}}\mathord{\cdotp }\infty . (\lambda y: {\mathbb{R}}\mathord{\cdotp }\infty . x + y)) 1 2 



